Trading Complexity for Sparsity in Random Forest Explanations

Random forests have long been considered as powerful model ensembles in machine learning. By training multiple decision trees, whose diversity is fostered through data and feature subsampling, the resulting random forest can lead to more stable and reliable predictions than a single decision tree. This however comes at the cost of decreased interpretability: while decision trees are often easily interpretable, the predictions made by random forests are much more difficult to understand, as they involve a majority vote over hundreds of decision trees. In this paper, we examine different types of reasons that explain "why" an input instance is classified as positive or negative by a Boolean random forest. Notably, as an alternative to sufficient reasons taking the form of prime implicants of the random forest, we introduce majoritary reasons which are prime implicants of a strict majority of decision trees. For these different abductive explanations, the tractability of the generation problem (finding one reason) and the minimization problem (finding one shortest reason) are investigated. Experiments conducted on various datasets reveal the existence of a trade-off between runtime complexity and sparsity. Sufficient reasons - for which the identification problem is DP-complete - are slightly larger than majoritary reasons that can be generated using a simple linear- time greedy algorithm, and significantly larger than minimal majoritary reasons that can be approached using an anytime P ARTIAL M AX SAT algorithm.

==> abstract.tex <==
\pierre{A compléter plus tard}

%Decision trees are popular ML models for the classification task because they are usually considered as highly interpretable.
%Indeed, for any instance to be classified using a decision tree, one can easily determine a subset of its characteristics that
%prove sufficient to explain the classification that is achieved. 
%
%Given a decision tree or a random forest, a sufficient reason of the instance to be classified, i.e., an irredundant subset of its 
%characteristics that proves sufficient to explain the classification that is achieved, 
%can be computed in polynomial time. However, such a sufficient reason is not guaranteed to be intelligible
%because it may contain too many characteristics. % and/or characteristics that are not comprehensible by the explainee.
%To deal with this issue, we focus on a refinement and on a generalization of the notion of sufficient reasons, namely the minimal reasons
%and the probable reasons, respectively.
%We identify the complexity of computing such reasons for a given instance when the classifier is a decision tree or a random forest, 
%and we describe exact or approximate algorithms for deriving them.  We also present
%empirical results for illustrating the gain in intelligibility they may offer and 
%the performances of the algorithms for computing them. 


==> additional.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Additional Results}\label{additional}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\paragraph{Minimal reasons.} Si on n'a pas la place on remet des paragraphes. Sinon les sous-section étant relativement longues, c'est plus lisible.

\subsection{Comprehensible Reasons}

%\paragraph{Comprehensible reasons.}  

Sufficient reasons are not always guaranteed to be ``intelligible''. 
Indeed, it can be the case that some features in the prime implicant 
are not understandable by the user to which the explanation is supplied. 
This calls for a notion of \emph{comprehensible reason}:

% Fred: l'exemple médical est intéressant, mais pas sûr qu'on ait la place.
% In some cases, limiting the size of an explanation to a few literals is not enough 
% to ensure that the explanation is intelligible \cite{CosteMarquis20}.
% Indeed, it can be the case that some of the features in the explanation are not understandable by the user to which the explanation
% must be reported. 
%This happens, for example, when trying to predict diseases from observed symptoms and physiological measures
%associated with patients: though the fact that the erythrocyte sedimentation rate in a blood test is over a given threshold is a
%meaningful piece of information for a physician, for many people this will be meaningless.

\begin{definition}[Comprehensible Reason] 
    Let $f \in \mathcal F_n$ and $\vec x \in \{0,1\}^n$ such that $f(\vec x) = 1$.
    In addition, let $I \subseteq X_n$ be a subset of intelligible features. 
    Then, a \emph{comprehensible reason} for $\vec x$ given $f$ and $I$ is a sufficient reason for $\vec x$ given $f$ that contains only literals built up from $I$.
\end{definition}

\begin{example} Suppose that the user does not understand what \emph{sympodial}\footnote{An orchid is sympodial when it grows sideways.} (feature $x_4$) means.
 Is it possible to find a sufficient reason for $\vec x$ given $T$ that does not include $x_4$? 
    Obviously, the answer is negative because $x_4$ is \emph{mandatory} for the {\it Cattleya} classifier $T$, that is, any sufficient reason 
    for any input instance must include a literal on $x_4$. 
\end{example}

As illustrated in the above example, a key issue for deriving ``intelligible'' reasons is to determine whether at least one comprehensible reason exists, 
depending on the choice of $I$. Interestingly, this problem is tractable for decision trees, and even for random forests: 

\begin{proposition} \label{prop:understandablereasonRF}
    Let $F \in \rf_{n, m}$ and $\vec x \in \{0,1\}^n$ such that $F(\vec x) = 1$. 
    Then, for any set $I \subseteq X_n$ of intelligible features, deciding whether a comprehensible reason for $\vec x$ given $F$ and $I$
    exists, and deriving such a reason when this is the case, can be done in $\mathcal O(n \size{F})$ time.
\end{proposition}

%\fred{Est-ce qu'on pourrait generaliser aux delta-probable comprehensible reasons? ... Cela reste poly, mais c'est une consequence de 3 \& 4.}
%\pierre{Oui, j'ai ajouté une phrase dans la partie "Probabilistic Reasons"}

%\color{blue}
%\pierre{J'ai remis la suite (partie en bleu). Merci de le mettre éventuellement en commentaires mais de ne pas l'effacer sinon cela m'oblige à retaper
%des trucs et je risque d'introduire des erreurs.}
%\fred{OK Pierre}

\subsection{Inclusion-Preferred Reasons}

%\fred{Pierre, si l'on a la place je suggere de mettre les raisons preferees au sens lexicographique (donc le modele LPM) 
%ainsi que les raisons preferees au sens lineaire additif (donc le modele APM). Sinon on se focalise sur LPM, où le resultat est poly. }

The user may also have some expectations about the features that should be present in explanations. 
For instance, she might consider that some features are more important than others for explaining decisions. 
The reason that is derived should cohere as much as possible to the user's expectations or \emph{confirmation bias}.\footnote{Confirmation bias is the tendency to search for, 
interpret, favor, and recall information in a way that confirms or supports one's prior beliefs or values. Since the 1960's, many experiments in psychology and cognitive science 
people have shown that people are biased toward confirming their existing beliefs (see e.g., \cite{Oswaldetal04}).}
However, when computing a sufficient reason, even a comprehensible one, we cannot guarantee that a ``better'' reason 
for the user would not exist. 

To make it more formal, one needs a notion of \emph{``preferred''} sufficient reason. Depending on the preference model at hand, the
computation of a single preferred reason can be intractable (as we will see soon). Fortunately, there are preference models for which
intractability can be avoided. 
 Especially, this is the case when the preference relation is ordinal and based on a total preorder $\leq$ over $X_n$,
 such that $x_i \leq x_j$ means that feature $x_i$ is considered as less important or less expected than feature $x_j$. 
 $\leq$ can be represented by a \emph{prioritization} (or stratification) of $X_n$, i.e., 
 an ordered partition $C_1, \ldots, C_p$ of the features from $X_n$ such that $x_i$ and $x_j$ belongs to the
 same set of the partition if and only if $x_i \leq x_j$ and $x_j \leq x_i$, and $C_i$ precedes $C_j$ in the partition (i.e., $i < j$) whenever
 every element of $C_i$ is before every element of $C_j$ w.r.t. $\leq$. Whatever $C$ among $C_1, \ldots, C_p$ and a term $t$ over $X_n$,
 $t[C]$ denotes the term composed of the literals of $t$ that are over variables from $C$.

 Based on the prioritization $C_1, \ldots, C_p$ of $X_n$ induced by $\leq$, one can define a preference relation $\sqsubset$ on the terms 
 over $X_n$ by stating that $t \sqsubset t'$ if and only if $\exists i \in \{1, \ldots, p\} \forall j \in \{1, \ldots, i-1\}$, $t[C_j] = t'[C_j]$ and 
 $t[C_i] \subset t'[C_i]$.\footnote{The construction is reminiscent to the one used for characterizing preferred subtheories in \cite{Brewka89}.}
 It can be checked that $\sqsubset$ is a strict, partial order (i.e., an irreflexive and transitive relation). 
 Given a set of terms, the minimal ones w.r.t. $\sqsubset$ correspond intuitively to those that contain as few unexpected literals
 as possible (where the comparison is based on set inclusion). On this ground, we are now ready to define the notion of inclusion-preferred reason:
 
\begin{definition}[Inclusion-Preferred Reason] 
    Let $f \in \mathcal F_n$, $\leq$ a total preorder over $X_n$, and $\vec x \in \{0,1\}^n$ be an instance such that $f(\vec x) = 1$.
    Then, an \emph{inclusion-preferred reason} for $\vec x$ given $f$ is a sufficient reason $t$ for $\vec x$ given $f$ 
    such that there is no sufficient reason $t'$ for $\vec x$ given $f$ satisfying $t' \sqsubset t$.
\end{definition}

\begin{example}[Example \ref{running-ex} cont'ed]
Suppose that the expectations of the explainee correspond to the prioritization $\{x_4\}, \{x_3, x_2\}, \{x_5\}, \{x_1\}$ reflecting the fact
that having fragrant flowers is, for her/him, a more salient aspect of {\it Cattleya} orchids than the other features.
% (especially than $d$ that she/he does not understand). 
Then $x_1 \wedge x_4$ is an inclusion-preferred reason for $\vec x$ given $T$, while $x_2 \wedge x_3 \wedge x_4$ is not because 
$x_1 \wedge x_4 \sqsubset x_2 \wedge x_3 \wedge x_4$ holds.
\end{example}

The greedy algorithm presented above for generating one sufficient reason can be cast in such a way that it generates
an inclusion-preferred reason for an instance given a decision tree, or more generally a random forest:

\begin{proposition} \label{prop:favoritereasonRF}
    Let $F \in \rf_{n,m}$, $\leq$ be a total preorder over $X_n$, and $\vec x \in \{0,1\}^n$. 
    Then, deriving an inclusion-preferred reason for $\vec x$ given $F$ and $\leq$ can be done in $\mathcal O(\size{G} + n \size{F})$ time
    where $G$ is the graph $(X_n, \leq)$.
\end{proposition}
%\color{black}

%\pierre{J'ai remis la suite comme elle était.}
%To make it more formal, one needs a notion of \emph{preferred} sufficient reason. Depending on the preference model at hand, the
%computation of a single preferred reason can be intractable. Fortunately, there are preference models for which
%intractability can be avoided. This is especially the case when preferences over features can be captured by a utility function 
%$u: X_n \rightarrow \R$, where $u(x_i) < u(x_j)$ indicates that $x_i$ is less preferred than $x_j$.\pierre{Euh, non, ce n'est pas traitable
%dans ce cas-là, on l'a montré avec les minimal reasons qui est un cas particulier de ``preferred reason'' où tous les $x_i$ ont des
%poids égaux non nuls. A revoir.}
%Based on this additive model, the utility of a term $t$ is given by $u(t) = \sum_{x_i \in \Var{t}} u(x_i)$.  
%
%\begin{definition}[Minimal-Weight Reason] 
%    Let $f \in \mathcal F_n$, $u: X_n \rightarrow \R$ be a utility function, and $\vec x \in \{0,1\}^n$ 
%    be an instance such that $f(\vec x) = 1$. Then, a \emph{minimal-weight reason} for $\vec x$ given $f$ is a sufficient reason 
%    $t$ for $\vec x$ given $f$ such that $u(t)$ is maximal.
%\end{definition}
%\pierre{J'appellerais plutôt cela des minimal-weight reasons pour garder ``preferred reason'' comme le terme générique. Je pense qu'il faut regrouper tout ce qui suit avec les minimal reasons
%car les minimal-weight reasons les généralisent et les algos exacts et approchés à base de partial-weighted-MAX-SAT s'appliquent de facon générale aux minimal-weight reasons si j'ai bien tout compris}
%\fred{*** Je m'arrete ici pour l'instant ***}

\subsection{Minimal Reasons}

As conciseness is often a desirable property of explanations, a natural way for improving the clarity of 
sufficient reasons is to focus on those of minimal size:

\begin{definition}[Minimal Reason] 
    Let $f \in \mathcal F_n$ and $\vec x \in \{0,1\}^n$ such that $f(\vec x) = 1$.
    A \emph{minimal reason} for $\vec x$ given $f$ is a sufficient reason for $\vec x$ given $f$ that contains a minimal number
    of literals.
\end{definition}

\begin{example} Based on our running example, $x_1 \wedge x_4$ is a minimal reason for $\vec x$ given $T$, 
    while $x_2 \wedge x_3 \wedge x_4$ is not.
\end{example}

Importantly, \emph{minimal reasons} should not to be confused with \emph{minimum-cardinality explanations}  \cite{ShihCD18},
where the minimality condition bears on the features set to $1$ in the input instance. 
%As a direct by-product of Proposition 8 from \cite{Audemardetal20}, 
%computing a minimum-cardinality explanation for an input instance $\vec x$ given a decision tree $T$
%can be done in polynomial-time. Unfortunately, this is not the case for minimal reasons, 
%which are computationally more demanding:
The computation of a minimal reason looks more demanding than the computation of a sufficient reason, even 
for the case of decision trees:

\begin{proposition}\label{prop:minimalreasonDT}
    Let $F \in \rf_{n,m}$ and $\vec x \in \{0,1\}^n$ such that $F(\vec x) = 1$.
%    Unless {\sf P = NP}, there is no polynomial-time algorithm for computing a minimal reason for $\vec x$ given $F$,
%    even when $F = \{T\}$ reduces to a single decision tree.
    Computing a minimal reason for $\vec x$ given $F$ is {\sf NP}-hard, 
    even when $F = \{T\}$ reduces to a single decision tree.
\end{proposition}

Obviously enough, this {\sf NP}-hardness result can be extended from minimal reasons to the more general concept of a minimal-weight reason.\footnote{A minimal 
reason is a minimal-weight reason whenever $w$ is a constant mapping from $X_n$ to $\mathbb{N}^*$.} 

\begin{definition}[Minimal-Weight Reason] 
    Let $f \in \mathcal F_n$ and $\vec x \in \{0,1\}^n$ such that $f(\vec x) = 1$. Let $w: X^n \rightarrow \mathbb{N}^*$ be a weight mapping
    associating with every feature a positive integer.
    A \emph{minimal-weight reason} for $\vec x$ given $f$ and $w$ is a sufficient reason $t$ for $\vec x$ given $f$ that minimizes
    $\Sigma_{x \in \Var{t}} w(x)$.
\end{definition}

$w$ can be interpreted as a cardinal preference over the features. When the explainee has such a preference in mind, it makes sense to lift it 
to terms (and reasons) by summing the weight (disutility) of the features occurring in the terms (and reasons).

Interestingly, computing a minimal-weight reason given a random forest and a weight mapping can be achieved by solving an instance of the
\textsc{Weighted Partial MaxSAT} problem:
%{\sf NP}-optimization problem:

\begin{proposition}\label{prop:minimaloptim}
    Let $F \in \rf_{n,m}$ and $\vec x \in \{0,1\}^n$ such that $F(\vec x) = 1$. Let $w: X^n \rightarrow \mathbb{N}^*$ be a weight mapping.
    A minimal-weight reason for $\vec x$ given $F = \{T_1, \ldots, T_m\}$ and $w$ consists of the literals shared by 
   $t_{\vec x} = \bigwedge_{i=1}^n \ell_i$ and  $t_{\vec v^*}$ where $\vec v^*$ is a solution of the instance of the 
   \textsc{Weighted Partial MaxSAT} problem given by the following multiset of weighted clauses:
   $$\{(\overline{x_i}, w(x_i)) \mid x_i(\vec x) = 1\} \cup \{(x_i, w(x_i)) \mid x_i(\vec x) = 0\}$$ 
   $$\cup \{(c, \infty) \mid c \in \cnf(\Sigma_{j=1}^m s_j > \frac{m}{2})\} \cup$$ 
   $$ \{(\overline{s_j} \vee c[\vec x], \infty) \mid  j \in [m] \mbox{ and } c \in \cnf(T_j)\}.$$
%    
%\noindent $\mathtt{Determine \: } \vec x^* \in \{0,1\}^n$\\
%\noindent $\mathtt{minimizing \: } \Sigma_{i=1}^n \mathit{sign}(\ell_i) \cdot w(x_i) \cdot x_i$\\
%\noindent $\mathtt{provided \: that}$\\
%\noindent $\Sigma_{j=1}^m s_j > \frac{m}{2}$\\
%\noindent $\overline{s_j} \vee c[\vec x] \mathtt{\: for \: every \: } j \in [m] \mathtt{\: and \: every \: } c \in \cnf(T_j)$
\end{proposition}

Let us recall that a \textsc{Weighted Partial MaxSAT} instance consists of a set of weighted clauses, where weights are
integers (the corresponding clauses are called soft clauses) or $\infty$ (the corresponding clauses are called hard clauses).
In the \textsc{Weighted Partial MaxSAT} instance presented in Proposition \ref{prop:minimaloptim}, $\cnf(\Sigma_{j=1}^m s_j > \frac{m}{2})$
denotes any \cnf\ encoding\footnote{Many such encodings exist, see \cite{DBLP:conf/cp/Sinz05,DBLP:journals/constraints/AsinNOR11}} of the cardinality constraint 
$\Sigma_{j=1}^m s_j > \frac{m}{2}$, where each $s_j$ ($j \in [m]$) is a selector variable associated with the decision tree $T_j$ of $F$. 
A solution of this instance is an assignment $\vec v^*$ of the variables occurring
in the clauses (here, variables from $X_n \cup \{s_j \mid j \in [m]\}$ plus the auxiliary variables used in the encoding of the cardinality constraint, if any)
that minimizes the sum of the weights of the clauses that are violated.

Interestingly, many algorithms for \textsc{Weighted Partial MaxSAT} have been designed during the past decade (see \cite{DBLP:journals/ai/AnsoteguiG17} 
for a presentation of the main ones). Thanks to Proposition \ref{prop:minimaloptim}, we can take advantage of them for computing minimal reasons and 
minimal-weight reasons.
%Based on this proposition, the task of finding minimal reasons can be encoded into a \textsc{Partial MaxSAT} problem.\pierre{Explain how or give a reference}
%Obviously enough, a \textsc{Partial MAX-SAT} algorithm for this task does not run in polynomial time in the worst case, 
%but due to the tremendous progress in \textsc{SAT} solving achieved during the past two decades since the advent of the CDCL architecture, 
%experiments show that, in practice, the algorithm finds minimal reasons in a reasonable amount of time (see Section \ref{experiments}). \pierre{Will see}

%Beyond minimal reasons, minimal-weight reasons can be computed by solving 
%Note that if a weight function $w$ associating with every characteristic $\ell_i$ of $t_{\vec x}$ was available,
%one could easily take advantage of it by replacing the objective function by $\Sigma_{i=1}^n \mathit{sign}(\ell_i) w(\ell_i) x_i$
%in the problem above. That way, we could compute a \emph{minimal-weight reason} for $\vec x$ given $F$, which can be better than
%a minimal reason from the explainee viewpoint given that it takes account for the preference relation between reasons captured
%by $w$.

%Nevertheless, both exact and approximation algorithms can be defined for the purpose of deriving a minimal reason
%by casting this task as a \textsc{Minimal Hitting Set} problem:
%
%\begin{proposition}\label{prop:MHS}
%    Let $T \in \dt_{n}$, and $\vec x \in \{0,1\}^n$ such that $T(\vec x) = 1$.
%    Let $H_{\vec x}(T)$ be the hypergraph formed by
%    the set of vertices $t_{\vec x}$ and the set of hyperedges $\{c \cap t_{\vec x}: c \in \cnf(T)\}$.
%    Then, $t$ is a minimal reason for $\vec x$ given $T$ if and only if $t$ is a minimal hitting set of $H_{\vec x}(T)$.
%\end{proposition}
%
%Based on this proposition, the task of finding minimal reasons can be encoded into a \textsc{Partial MAX-SAT} problem,
%where the collection of hard clauses (which must be satisfied) is the set of hyperedges in $H_{\vec x}(T)$, and the 
%set of soft clauses (which can be violated) is $\{\neg l_i : l_i \in t_{\vec x}\}$.
%Obviously enough, a \textsc{Partial MAX-SAT} algorithm for this task does not run in polynomial time in the worst case, 
%but due to the tremendous progress in \textsc{SAT} solving achieved during the past two decades since the advent of the CDCL architecture, 
%experiments show that, in practice, the algorithm finds minimal reasons in a reasonable amount of time (see Section \ref{experiments}). 
%\footnote{The existence of such an algorithm would prove {\sf P = NP}.} -> Pour IJCAI, on n'a pas vraiment besoin de le préciser :-)

As an alternative to \textsc{Weighted Partial MaxSAT} solving, we can find good approximations of minimal reasons using the following greedy covering algorithm:
starting from $t = \emptyset$, iteratively add to $t$ a vertex $l_i \in t_{\vec x}$ of maximal degree $\mathrm{deg}(l_i)$, and removes it together with all 
adjacent hyperedges in $H_{\vec x}(T)$. Let $\mathrm{adj}(l_i)$ be the set of vertices in $H_{\vec x}(T)$ which are adjacent to $l_i$, 
and let $A = \max_{i=1}^n \size{\mathrm{adj}(l_i)}$. Note that for the \cnf\ encoding of decision trees, 
$A$ often coincides with the depth of the tree. Based on the analysis of greedy covering algorithm \cite{SLAVIK1997,OKUN2005}, we get the following result. 

\begin{proposition}\label{prop:approximable}
    Given $T \in \dt_{n}$ and $\vec x \in \{0,1\}^n$ such that $T(\vec x) = 1$, the problem of finding 
    a minimal reason for $\vec x$ with respect to $T$ is approximable to within a ratio of $\min(A/2 + 1, \ln n - \ln\ln n + \Theta(1))$. 
\end{proposition}

Unfortunately, this result does not extend to the case of random forests. \pierre{Write a proposition that states it formally}

Finally, a direct consequence of Proposition \ref{prop:minimalreasonDT} is that the greedy algorithm used for pointing out in polynomial time a sufficient reason 
cannot be extended to the issue of selecting a ``preferred'' reason from the sufficient ones when any preference relation is considered. 
%Especially, as we will see next, computing a reason that contains as few features
%as possible cannot be achieved in polynomial time unless {\sf P = NP}. The search for a ``preferred reason''
%among the sufficient reasons cannot always be done efficiently. 
Note that a straightforward generate-and-test algorithm would not be not
convenient to reach the goal because the search space (i.e., the set of all sufficient reasons) is of exponential size
in the worst case.
%For the classes of \cnf\ and \dnf\ formulas, it is well-known that an input instance can have exponentially many sufficient reasons.
%For example, the monotone \cnf\ formula $F = \bigwedge_{i=1}^{\lfloor\frac{n}{2}\rfloor} (x_{2i-1} \vee x_{2i})$ has $2^{\lfloor\frac{n}{2}\rfloor}$.
%prime implicants, each of them being implied by $\vec x = (1,1,\cdots,1)$. Surprisingly, 
Indeed, even for the restricted class of decision trees of 
logarithmic depth, an input instance can have exponentially many sufficient reasons:

\begin{proposition}\label{prop:nbDT}
    Let $\dt^k_{n}$ be the class of decision trees of depth $k \geq 1$ over $n = 2^k - 1$ variables. Then, there is a decision tree $T \in \dt^k_{n}$ 
    such that for any $\vec x \in \{0,1\}^n$, the number of sufficient reasons for $\vec x$ given $T$ is at least $\lfloor \frac{3}{2}^{\frac{n + 1}{2}} \rfloor$. 
\end{proposition}

%\paragraph{Probabilistic Reasons.} 

\subsection{Probabilistic Reasons}

A natural way to circumvent the computational barrier of finding minimal reasons is to rely on a probabilistic notion of prime implicant explanations,
as suggested in \cite{WALDCHEN2020}. This leads to generalize the notion of sufficient reasons, instead of refining it.
Basically, the idea of ``probabilistic`'' prime implicants stems from the fact that standard, ``logical'' prime implicants 
are often too rigid for high dimensional, and possibly noisy, classification tasks. Thus, by forgetting few models of the classifier $f$, 
probabilistic prime implicants may provide much shorter explanations. Formally, let $\PP_{\vec z}[f(\vec z)]$ be the probability 
that an assignment $\vec z$, drawn at random according to the uniform distribution over $\{0,1\}^n$, is a model of $f$, i.e.
\begin{align*}
\PP_{\vec z}[f(\vec z)] = \frac{\size{\vec z \in \{0,1\}^n: f(\vec z) = 1}}{\size{\vec z \in \{0,1\}^n}}
\end{align*}
Now, let $\PP_{\vec z}[f(\vec z) \mid t \subseteq t_{\vec z}]$ be the conditional probability that a random assignment $\vec z$ is a model of $f$, 
given that $\vec z$ is an extension of $t$:
\begin{align*}
   \PP_{\vec z}[f(\vec z) \mid t \subseteq t_{\vec z}] = \frac{\size{\vec z \in \{0,1\}^n: f(\vec z) = 1 \mbox{ and } t \subseteq t_{\vec z}}}{\size{\vec z \in \{0,1\}^n: t \subseteq t_{\vec z}}}
\end{align*}
For a confidence parameter $\delta \in [0, 1]$, a term $t$ is called a $\delta$-\emph{probable implicant} of $f$ if $\PP_{\vec z}[f(\vec z) \mid t \subseteq t_{\vec z}] \geq \delta$, 
that is, the proportion of extensions of $t$ that are models of $f$ is at least $\delta$. If $t$ is a $\delta$-probable implicant of $f$ and no proper subset of $t$ 
is a $\delta$-probable implicant of $f$, then $t$ is called a $\delta$-\emph{probable prime implicant} of $f$.

\begin{definition}[$\delta$-Probable Reason] 
    Let $f \in \mathcal F_n$ and $\vec x \in \{0,1\}^n$ such that $f(\vec x) = 1$.
    A \emph{$\delta$-probable reason} for $\vec x$ given $f$ is a $\delta$-probable prime implicant $t$ of $f$ such that $t \subseteq t_{\vec x}$.
\end{definition}

\begin{example}
    Based on our running example, we can observe that $x_2 \land x_4$ is not a sufficient reason for $\vec x$ given $T$, but it is
    still a $75\%$-probable reason for $\vec x$ (given $T$).
\end{example}
    
Clearly enough, considering $\delta$-probable reasons can also be a way to get rid of incomprehensible characteristics in sufficient reasons
(even if there is no guarantee that incomprehensible characteristics are systematically removed).

% \begin{definition}[Approximate Implicant]
% Let $\delta \in [0, 1]$. A term $t$ is a $\delta$-\emph{approximate implicant} of a Boolean function $f \in \mathcal F_n$ if and only if
% $f \mid t$ has a number of models (over its set of variables) that is $\geq \delta \times 2^{|\mathit{Var}(f \mid t)|} $.
% \end{definition}
% Thus, any term is a $0$-approximate implicant of $f$ and the implicants $t$ of $f$ are precisely the 
% $1$-approximate implicants of $\Sigma$.
% On this basis, we can easily define a notion of approximate reason:
%
%\begin{definition}[prime approximate implicant]
%Let $\delta \in [0, 1]$. A term $\gamma$ is a \emph{prime} $\delta$-\emph{approximate implicant} of a Boolean function $\Sigma$ if and only if
%$\gamma$ is a $\delta$-approximate implicant of $\Sigma$, and $\gamma$ deprived of any of its literal $\ell$ is not a $\delta$-approximate 
%implicant of $\Sigma$.
%\end{definition}
% \begin{definition}[Approximate Reason]
% Let $\delta \in [0, 1]$. 
% \begin{itemize}
% \item A term $t$ is a \emph{prime} $\delta$-\emph{approximate implicant} of a Boolean function $f \in \mathcal F_n$ if and only if
% $t$ is a $\delta$-approximate implicant of $f$, and $t$ deprived of any of its literal $\ell$ is not a $\delta$-approximate 
% implicant of $f$.
% \item A term $t$ is an $\delta$-\emph{approximate reason} for an instance $\vec{x} \in \{0,1\}^n$  given a Boolean function $f \in \mathcal F_n$ if and only if
% $t$ is a prime $\delta$-approximate implicant of $f$ such that $\vec{x} \models t$ holds.
% \end{itemize}
% \end{definition}
% Note that focusing on $\delta$-\emph{approximate reasons} instead of sufficient reasons not only is a way to get shorter (thus more intelligible)
% explanations, but also to get rid of mandatory features that can be unintelligible by the explainee.

Finding $\delta$-probable reasons is an ${\sf NP^{PP}}$-\pierre{hard} problem (see Theorem 2.4 in \cite{WALDCHEN2020}). 
However, this problem can be shown as tractable for decision trees via slightly modifying the greedy algorithm for sufficient reasons. Namely, at each iteration $i \in [n]$, 
instead of testing whether the current term $t$, deprived from the literal $l_i$, is an implicant of $T$, we check whether $t \setminus \{l_i\}$ is a $\delta$-probable implicant 
of $T$. Using the fact that conditioning and model counting operations can be done in linear time for decision trees \cite{Koricheetal13}, the inequality 
$\PP_{\vec z}[f(\vec z) \mid t \subseteq t_{\vec z}] \geq \delta$ can be checked in linear time. %To sum up:

\begin{proposition}\label{prop:probabilisticreasonDT}
Let $T \in \dt_n$ and $\vec{x} \in \{0,1\}^n$ such that $T (\vec{x}) = 1$.
Then, finding a $\delta$-probable reason for $\vec x$ given $T$ can be done in $O(n\size{T})$ time.
\end{proposition}

Unfortunately, this result cannot be extended to the case of random forests:

\begin{proposition}\label{prop:probabilisticreasonRF}
    Let $F \in \rf_{n,m}$ and $\vec x \in \{0,1\}^n$ such that $F(\vec x) = 1$.
%    Unless {\sf P = NP}, there is no polynomial-time algorithm for computing a $\delta$-probable reason for $\vec x$ given $F$.
 Computing a $\delta$-probable reason for $\vec x$ given $F$ is {\sf \#P}-hard.
\end{proposition}

% From this proposition, we can easily design a polynomial-time greedy algorithm for deriving a $\delta$-approximate reason 
% for any instance $\vec{x}$ given a decision tree $T$ (this algorithm is very close to the one used for deriving a sufficient reason, which
% is sketched above).
%sketched in the proof of Proposition \ref{prop:onesufficientRF}).


==> alternative.tex <==
\color{black}

\newpage

\fred{Preuves alternatives exploitant les resultats de Judy Goldsmith et ceux de Christopher Umans.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Some Alternative Results} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Sufficient Reasons}

We first consider sufficient reasons for arbitrary propositional formulas.

\begin{center}
\fcolorbox{black}{white}
{
\begin{minipage}{0.98\textwidth}
    \textsc{Is Prime Implicant (IPI)}
    \begin{itemize}
    \item \emph{Instance:} A Boolean formula $F$ and a monomial $t$.
    \item \emph{Question:} Is $t$ a prime implicant of $F$?
    \end{itemize}    
\end{minipage}
}
\end{center}
\vspace{0.5em}

\begin{proposition}
\textsc{Is Prime Implicant} is \textsf{DP}-complete.
\end{proposition}
\begin{proof}
Directly follows from Theorem 5 in \cite{Goldsmith2008}.
\end{proof}

\begin{center}
    \fcolorbox{black}{white}
    {
    \begin{minipage}{0.98\textwidth}
        \textsc{Is Sufficient Reason (ISR)}
        \begin{itemize}
        \item \emph{Instance:} A Boolean formula $F$, an assignment $\vec x$, and a monomial $t$.
        \item \emph{Question:} Is $t$ a sufficient reason of  $\vec x$ given $F$?
        \end{itemize}    
    \end{minipage}
    }
\end{center}
\vspace{0.5em}
    
\begin{proposition}
    \label{prop:ISR}
\textsc{Is Sufficient Reason} is \textsf{DP}-complete.
\end{proposition}
\begin{proof}
The membership part follows from the fact that ISR is a special case of IPI.
For the hardness part, consider an instance $(F,t)$ of IPI, and let $(F,\vec x,t)$ be the corresponding 
instance of ISR, where $\vec x$ is any assignment covered by $t$. Obvisouly, 
$(F,\vec x,t)$ can be constructed in linear time. 
Now, if $(F,t)$ is a solution of IPI, then $t$ is a prime implicant of $F$. This, 
together with the fact that $t$ covers $\vec x$ implies that $(F,\vec x,t)$ is a solution of ISR.
Conversely, if $(F,\vec x,t)$ is a solution of ISR, then $t$ is a a prime implicant of $F$, 
which immediately implies that $(F,t)$ is a solution of IPI.  
\end{proof}

We now consider the subclass of DNF formulas.

\begin{center}
    \fcolorbox{black}{white}
    {
    \begin{minipage}{0.98\textwidth}
        \textsc{Is DNF Prime Implicant (IPI[DNF])}
        \begin{itemize}
        \item \emph{Instance:} A DNF formula $F$ and a monomial $t$.
        \item \emph{Question:} Is $t$ a prime implicant of $F$?
        \end{itemize}    
    \end{minipage}
    }
\end{center}
\vspace{0.5em}

\begin{proposition}
    \textsc{Is DNF Prime Implicant} is \textsf{DP}-complete.
\end{proposition}
    \begin{proof}
        Follows from Theorem 6.7 in \cite{Umans2006}.
    \end{proof}
    
    \begin{center}
        \fcolorbox{black}{white}
        {
        \begin{minipage}{0.98\textwidth}
            \textsc{Is DNF Sufficient Reason (ISR[DNF])}
            \begin{itemize}
            \item \emph{Instance:} A DNF formula $F$, an assignment $\vec x$, and a monomial $t$.
            \item \emph{Question:} Is $t$ a sufficient reason of  $\vec x$ given $F$?
            \end{itemize}    
        \end{minipage}
        }
    \end{center}
    \vspace{0.5em}

\begin{proposition}
        \textsc{Is DNF Sufficient Reason} is \textsf{DP}-complete.
        \end{proposition}
        \begin{proof}
          Straightforward, using a strategy similar to the proof of Proposition \ref{prop:ISR}.  
        \end{proof}

With these results in hand, let us turn to our problem.

\begin{center}
    \fcolorbox{black}{white}
    {
    \begin{minipage}{0.98\textwidth}
        \textsc{Is Sufficient Reason for Random Forests (ISR[RF])}
        \begin{itemize}
        \item \emph{Instance:} A random forest $F$, an assignment $\vec x$, and a monomial $t$.
        \item \emph{Question:} Is $t$ a sufficient reason of  $\vec x$ given $F$?
        \end{itemize}    
    \end{minipage}
    }
\end{center}
\vspace{0.5em}

\begin{proposition}
\textsc{Is Sufficient Reason for Random Forests} is \textsf{DP}-complete.
\end{proposition}
\begin{proof}
    The membership part follows from the fact that ISR[RF] is a special case of ISR, and the hardness 
    part follows from the fact that ISR[DNF] is a special case of ISR[RF].
\end{proof}

\newpage
    
%\subsection{Minimal Reasons}


%For illustration, the following toy example will be used throughout the paper as a running example:


% Deciding whether any term $t$ included in $\vec x$ is an implicant of $T$ is equivalent to checking whether 
% $t$ entails $\cnf(T)$, which can be done in $O(\size{T})$ time. 
% Thus, by performing this implicant test $n$ times, the runtime of the greedy algorithm is in $\mathcal O(\size{T}n)$.

% The key task of the greedy algorithm is to decide whether any term $t$ included in $\vec x$  is an 
% implicant of $T$, which is equivalent to check whether $T \mid t$ (the conditioning of $T$ by $t$) 
% is a decision tree with no leaves labeled by $0$. To this point, $T \mid t$ can be constructed in $O(\size{T})$
% time using the following procedure: sort all internal vertices of $T$ in reverse topological order and, 
% for each vertex $v_i$ in that order, check whether the corresponding variable $x_i$ 
% occurs as a literal $l_i$ of $t$\footnote{This can be done in $\mathcal O(1)$ time using a vector encoding of $t$.}. 
% If so, replace the node $v_i$ by its right child if $l_i = x_i$, and its left child if $l_i = \overline x_i$.
% By performing this implicant test $n$ times, the runtime of the greedy algorithm is in $\mathcal O(\size{T}n)$.

% which returns as output a sufficient reason $t$ for $\vec x$ given $T$ in $\mathcal O(n \size{T})$ time.
% \footnote{Note that this algorithm can be extended easily to the case of random forests without questioning its tractability.}
% The tractability of finding sufficient reasons in decision trees lies in the fact that deciding whether a consistent term $t$ is an implicant 
% of a decision tree $T$ can be obtained by checking whether $T \mid t$ (the conditioning of $T$ by $t$) 
% is a decision tree with no leaves labeled by $0$. Notably, $T \mid t$ can be computed in $\mathcal O(\size{T} \size{t})$ 
% time by iteratively conditioning $T$ by each literal occurring in $t$. For any such literal $l_i$ with variable $x_i$,
% $T \mid l_i$ is obtained by simply replacing each internal node $x_i$ in $T$ with its right child if $l_i = x_i$, 
% and its left child if $l_i = \overline x_i$.
    % With this implicant test in hand, the generation of a sufficient reason for $\vec x$ given $T$ 
% can be found using the following greedy algorithm: start with $t = \vec x$, and iterate over the literals $l_i$ of 
% $t$ by checking whether $t$ deprived of $l_i$ is still an implicant of $T$. 
% If so, remove $l_i$ from $t$ and proceed to the next literal.
% Once all the variables $\vec{x}$ have been examined, the term $t$ is by construction an implicant of $T$ such that
% removing any literal from $t$ would lead to a term that is not any longer an implicant of $T$. Thus, $t$
% is a prime implicant of $T$ and it contains only literals from $\vec{x}$.


% Deciding whether any term $t$ included in $\vec x$ is an implicant of $T$ is equivalent to checking whether 
% $t$ entails $\cnf(T)$, which can be done in $O(\size{T})$ time. 
% Thus, by performing this implicant test $n$ times, the runtime of the greedy algorithm is in $\mathcal O(\size{T}n)$.

% The key task of the greedy algorithm is to decide whether any term $t$ included in $\vec x$  is an 
% implicant of $T$, which is equivalent to check whether $T \mid t$ (the conditioning of $T$ by $t$) 
% is a decision tree with no leaves labeled by $0$. To this point, $T \mid t$ can be constructed in $O(\size{T})$
% time using the following procedure: sort all internal vertices of $T$ in reverse topological order and, 
% for each vertex $v_i$ in that order, check whether the corresponding variable $x_i$ 
% occurs as a literal $l_i$ of $t$\footnote{This can be done in $\mathcal O(1)$ time using a vector encoding of $t$.}. 
% If so, replace the node $v_i$ by its right child if $l_i = x_i$, and its left child if $l_i = \overline x_i$.
% By performing this implicant test $n$ times, the runtime of the greedy algorithm is in $\mathcal O(\size{T}n)$.

% which returns as output a sufficient reason $t$ for $\vec x$ given $T$ in $\mathcal O(n \size{T})$ time.
% \footnote{Note that this algorithm can be extended easily to the case of random forests without questioning its tractability.}
% The tractability of finding sufficient reasons in decision trees lies in the fact that deciding whether a consistent term $t$ is an implicant 
% of a decision tree $T$ can be obtained by checking whether $T \mid t$ (the conditioning of $T$ by $t$) 
% is a decision tree with no leaves labeled by $0$. Notably, $T \mid t$ can be computed in $\mathcal O(\size{T} \size{t})$ 
% time by iteratively conditioning $T$ by each literal occurring in $t$. For any such literal $l_i$ with variable $x_i$,
% $T \mid l_i$ is obtained by simply replacing each internal node $x_i$ in $T$ with its right child if $l_i = x_i$, 
% and its left child if $l_i = \overline x_i$.
    % With this implicant test in hand, the generation of a sufficient reason for $\vec x$ given $T$ 
% can be found using the following greedy algorithm: start with $t = \vec x$, and iterate over the literals $l_i$ of 
% $t$ by checking whether $t$ deprived of $l_i$ is still an implicant of $T$. 
% If so, remove $l_i$ from $t$ and proceed to the next literal.
% Once all the variables $\vec{x}$ have been examined, the term $t$ is by construction an implicant of $T$ such that
% removing any literal from $t$ would lead to a term that is not any longer an implicant of $T$. Thus, $t$
% is a prime implicant of $T$ and it contains only literals from $\vec{x}$.
%
%Finally, it is worth noting that the problem of deriving \emph{all} sufficient reasons for
%a given instance is much more demanding in general. Indeed, even for the restricted class of decision trees with
%logarithmic depth, an input instance can have exponentially many sufficient reasons:
%
%\begin{proposition}\label{prop:nbDT}
%%    Let $\dt^k_{n}$ be the class of decision trees of depth $k \geq 1$ over $n = 2^k - 1$ variables. Then, t
%There is a decision tree $T$ of depth $k \geq 1$ over $n = 2^k - 1$ variables
% such that for any $\vec x \in \{0,1\}^n$, the number of sufficient reasons for $\vec x$ given $T$ is at least 
% $\lfloor \frac{3}{2}^{\frac{n + 1}{2}} \rfloor$. 
%\end{proposition}


==> beyond.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Beyond Sufficient Reasons}\label{beyond}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Minimal Reasons}

As conciseness is often a desirable property of explanations, a natural way for improving the clarity of 
sufficient reasons is to focus on those of minimal size:

\begin{definition}[Minimal Reason] 
    Let $f \in \mathcal F_n$ and $\vec x \in \{0,1\}^n$ such that $f(\vec x) = 1$.
    A \emph{minimal reason} for $\vec x$ given $f$ is a sufficient reason for $\vec x$ given $f$ that contains a minimal number
    of literals.\footnote{Minimal reasons should not to be confused with \emph{minimum-cardinality explanations}  \cite{ShihCD18},
    where the minimality condition bears on the features set to $1$ in the input instance.}
\end{definition}

\begin{example} For our running example, $x_1 \wedge x_4$ is the unique minimal reason for $\vec x$ given $F$.
 %   while $x_2 \wedge x_3 \wedge x_4$ is not.
\end{example}

Given Proposition \ref{prop:sufficient reason-MUS-RF}, a minimal reason for $\vec x$ given $f$ can be characterized as a {\it minimal MUS}. Thus, one can
take advantage of algorithms for computing minimal MUSes in order to derive minimal reasons. \pierre{Ajouter des réfs}
However, deriving a minimal reason is computationally harder 
than deriving a sufficient reason:

\begin{proposition}\label{prop:complexityminimalMUS}
    Let $f \in \mathcal F_n$ and $\vec x \in \{0,1\}^n$ such that $f(\vec x) = 1$.
    Deciding whether there exists a minimal reason $t$ for $\vec x$ given $f$ such that $t$ contains at most $k$ features is $\Sigma_2^p$-complete.
\end{proposition}

As a by-product of Proposition \ref{prop:complexitysufficientreasonRF}, leveraging an algorithm for computing a minimal MUS in order to
compute a minimal reason looks as a reasonable approach because both problems have the same complexity 
(deciding whether there exists a MUS $I$ of $S$ given $H$ that contains at most $k$ literals also is $\Sigma_2^p$-complete).

%\pierre{Revoir toute la suite : les résultats que l'on avait concernaient en fait des proto-sufficient reasons. Voir si l'on a besoin d'introduire les proto-sufficient reasons, i.e., les termes qui sont des raisons suffisantes pour $\vec x$ étant donné $T$ pour une majorité d'arbres $T$ dans $F$ ? Pas sûr que l'on en ait besoin. Eventuellement comme leur calcul peut être réalisé par des algos plus efficaces - en temps polynomial - comparé aux sufficient reasons), on pourra les garder au cas où cela se passe mal expérimentalement avec les MUS. Cela donne un compromis entre l'efficacité du calcul et la qualité de l'explication.}


%Arguably, the task of finding minimal reasons shares similarities with the \textsc{Shortest Implicant} problem, 
%in which we are given a representation of a Boolean function $f$ together with an integer $k$,
%and the goal is to find an implicant $t$ of $f$ that contains at most $k$ literals. This problem is known to be $\mathsf{\Sigma_2^p}$-hard
%for \dnf\ formulae \cite{DBLP:journals/jcss/Umans01}, and by direct application of Proposition~\ref{prop:CNF2RF}, it is $\mathsf{\Sigma_2^p}$-hard for random forests. 
%Yet, there is a subtle difference with the problem of finding a minimal reason for an instance $\vec x$ given $f$.
%Here, the target implicant $t$ \emph{must cover} $\vec x$, as it captures an explanation for $f(\vec x) = 1$. 
%The computational complexity this problem is slightly less demanding: 


%As a direct by-product of Proposition 8 from \cite{Audemardetal20}, 
%computing a minimum-cardinality explanation for an input instance $\vec x$ given a decision tree $T$
%can be done in polynomial-time. Unfortunately, this is not the case for minimal reasons, 
%which are computationally more demanding:
% The computation of a minimal reason looks more demanding than the computation of a sufficient reason, even 
% for the case of decision trees:

%\begin{proposition}\label{prop:minimalreasonDT}
%    Let $F \in \rf_{n,m}$, $\vec x \in \{0,1\}^n$ such that $F(\vec x) = 1$, and $k \in \mathbb N$.
%    Then, finding a minimal reason for $\vec x$ given $F$ of size at most $k$ is {\sf NP}-complete,
%    even when $m = 1$.
%\end{proposition}
%
%A common approach for efficiently handling this issue is to rely on modern constraint solvers, 
%by casting the task of finding minimal reasons as a Boolean constraint optimization problem. 
%To this end, recall that a \textsc{Partial MaxSAT} problem consists in a pair  $(C_{\mathrm{soft}}, C_{\mathrm{hard}})$
%of \cnf\ formulas, and the goal is to find a Boolean assignment that satisfies a maximum number of 
%clauses in $C_{\mathrm{soft}}$, while satisfying all clauses in $C_{\mathrm{hard}}$.
%
%\begin{proposition}\label{prop:minimaloptim}
%    Let $F = \{T_1,\cdots,T_m\}$ be a random forest in $\rf_{n,m}$ and $\vec x \in \{0,1\}^n$ be an instance such that $F(\vec x) = 1$. 
%    Let $(C_{\mathrm{soft}}, C_{\mathrm{hard}})$ be an instance of the \textsc{Partial MaxSAT} problem such that:
%    \begin{align*}
%        C_{\mathrm{soft}} &= \{\overline x_i  : x_i \in t_{\vec x}\} \cup \{x_i  : \overline x_i \in t_{\vec x}\} \\
%        C_{\mathrm{hard}} &= \cnf\left(\sum_{j = 1}^m y_j > \frac{m}{2} \right) \\
%        &\quad \cup \{( \overline y_j \vee c_{\mid \vec x}) : j \in [m], c \in \cnf(T_j) \} 
%    \end{align*}
%    where $c_{\mid \vec x} = c \cap t_{\vec x}$ is the restriction of $c$ to the literals in $t_{\vec x}$.
%    Then, any optimal solution of $(C_{\mathrm{hard}}, C_{\mathrm{soft}})$ projected on the literals over $X_n$ is 
%    a minimal reason for $\vec x$ given $F$.
%\end{proposition}
%
%In the above proposition, the constraint $\smash{\cnf(\Sigma_{j=1}^m y_j > \frac{m}{2})}$ denotes any \cnf\ encoding\footnote{Many such encodings exist, see \cite{DBLP:conf/cp/Sinz05,DBLP:journals/constraints/AsinNOR11}} of the cardinality constraint 
%$\Sigma_{j=1}^m y_j > \frac{m}{2}$, where each $y_j$ ($j \in [m]$) is a selector variable associated with the decision tree $T_j$ of $F$. 

%A solution of this instance is an assignment $\vec v^*$ of the variables occurring
%in the clauses (here, variables from $X_n \cup \{y_j \mid j \in [m]\}$ plus the auxiliary variables used in the encoding of the cardinality constraint, if any)
%that minimizes the sum of the weights of the clauses that are violated. 
%Interestingly, many algorithms for \textsc{Weighted Partial MaxSAT} have been designed during the past decade (see \cite{DBLP:journals/ai/AnsoteguiG17} 
%for a presentation of the main ones). Thanks to Proposition \ref{prop:minimaloptim}, we can take advantage of them for computing minimal reasons and 
%minimal-weight reasons.
%Based on this proposition, the task of finding minimal reasons can be encoded into a \textsc{Partial MaxSAT} problem.\pierre{Explain how or give a reference}
%Obviously enough, a \textsc{Partial MAX-SAT} algorithm for this task does not run in polynomial time in the worst case, 
%but due to the tremendous progress in \textsc{SAT} solving achieved during the past two decades since the advent of the CDCL architecture, 
%experiments show that, in practice, the algorithm finds minimal reasons in a reasonable amount of time (see Section \ref{experiments}). \pierre{Will see}

%Beyond minimal reasons, minimal-weight reasons can be computed by solving 
%Note that if a weight function $w$ associating with every characteristic $\ell_i$ of $t_{\vec x}$ was available,
%one could easily take advantage of it by replacing the objective function by $\Sigma_{i=1}^n \mathit{sign}(\ell_i) w(\ell_i) x_i$
%in the problem above. That way, we could compute a \emph{minimal-weight reason} for $\vec x$ given $F$, which can be better than
%a minimal reason from the explainee viewpoint given that it takes account for the preference relation between reasons captured
%by $w$.

%Nevertheless, both exact and approximation algorithms can be defined for the purpose of deriving a minimal reason
%by casting this task as a \textsc{Minimal Hitting Set} problem:
%
%\begin{proposition}\label{prop:MHS}
%    Let $T \in \dt_{n}$, and $\vec x \in \{0,1\}^n$ such that $T(\vec x) = 1$.
%    Let $H_{\vec x}(T)$ be the hypergraph formed by
%    the set of vertices $t_{\vec x}$ and the set of hyperedges $\{c \cap t_{\vec x}: c \in \cnf(T)\}$.
%    Then, $t$ is a minimal reason for $\vec x$ given $T$ if and only if $t$ is a minimal hitting set of $H_{\vec x}(T)$.
%\end{proposition}
%
%Based on this proposition, the task of finding minimal reasons can be encoded into a \textsc{Partial MAX-SAT} problem,
%where the collection of hard clauses (which must be satisfied) is the set of hyperedges in $H_{\vec x}(T)$, and the 
%set of soft clauses (which can be violated) is $\{\neg l_i : l_i \in t_{\vec x}\}$.
%Obviously enough, a \textsc{Partial MAX-SAT} algorithm for this task does not run in polynomial time in the worst case, 
%but due to the tremendous progress in \textsc{SAT} solving achieved during the past two decades since the advent of the CDCL architecture, 
%experiments show that, in practice, the algorithm finds minimal reasons in a reasonable amount of time (see Section \ref{experiments}). 
%\footnote{The existence of such an algorithm would prove {\sf P = NP}.} -> Pour IJCAI, on n'a pas vraiment besoin de le préciser :-)

%As an alternative to \textsc{Partial MaxSAT} solving, we may explore the possibility of finding good approximations of minimal reasons 
%in polynomial-time. For decision trees, this task can be cast as a \textsc{Min Hitting Set} problem: given a representation $T \in \dt_n$ 
%and an instance $\vec x \in \{0,1\}^n$ such that $T(\vec x) = 1$, let $H_{\vec x}(T)$ be the hypergraph formed by
%the set of vertices $t_{\vec x}$ and the set of hyperedges $\{c_{\mid \vec x} : c \in \cnf(T)\}$.
%By construction, $t$ is a minimal reason for $\vec x$ given $T$ if and only if $t$ is a minimal hitting set of $H_{\vec x}(T)$.
%Based on this equivalence, one can use the well-known greedy algorithm for \textsc{Min Hitting Set} which achieves a logarithmic approximation ratio \cite{SLAVIK1997,OKUN2005}.

For decision trees, it is possible to find good approximations of minimal reasons in polynomial-time \cite{ref-our-paper-submitted-to-ijcai21}.
For random forests, approximating minimal reasons is much harder mainly due to the fact that, by Proposition~\ref{prop:CNF2RF}  
any \cnf\ formula can be transformed into an equivalent \rf. Thus: 

% of minimal reasons using the following greedy covering algorithm:
% starting from $t = \emptyset$, iteratively add to $t$ a vertex $l_i \in t_{\vec x}$ of maximal degree $\mathrm{deg}(l_i)$, and removes it together with all 
% adjacent hyperedges in $H_{\vec x}(T)$. Let $\mathrm{adj}(l_i)$ be the set of vertices in $H_{\vec x}(T)$ which are adjacent to $l_i$, 
% and let $A = \max_{i=1}^n \size{\mathrm{adj}(l_i)}$. Note that for the \cnf\ encoding of decision trees, 
% $A$ often coincides with the depth of the tree. Based on the analysis of greedy covering algorithm \cite{SLAVIK1997,OKUN2005}, we get the following result. 

\begin{proposition}\label{prop:approximable}
    Let $F \in \rf_{n,m}$, and $\vec x \in \{0,1\}^n$ such that $F(\vec x) = 1$. 
%    If $f$ is a decision tree in $\dt_n$ then finding a minimal reason for $\vec x$ given $f$ 
%    is approximable to within a ratio of $\ln n - \ln\ln n + \Theta(1)$. On the other hand, if $f$ 
%    is an arbitrary random forest in $\rf_{n,m}$, then finding a minimal reason for $\vec x$ given $f$ is not 
%    approximable to within any factor.
%    
    Finding a minimal reason for $\vec x$ given $F$ is not approximable to within any factor.
\end{proposition}

\pierre{Il manque la preuve de ce résultat.}

%\fred{En utilisant la reduction via MINONES on peut montrer que c'est polyAPX, mais je conjecture qu'on est encore plus haut ! 
%Donc je bosse encore un peu dessus.}

%Finally, a direct consequence of Proposition \ref{prop:minimalreasonDT} is that the greedy algorithm used for pointing out in polynomial time a sufficient reason 
%cannot be extended to the issue of selecting a ``preferred'' reason from the sufficient ones when any preference relation is considered. 
%%Especially, as we will see next, computing a reason that contains as few features
%%as possible cannot be achieved in polynomial time unless {\sf P = NP}. The search for a ``preferred reason''
%%among the sufficient reasons cannot always be done efficiently. 
%Note that a straightforward generate-and-test algorithm would not be not
%convenient to reach the goal because the search space (i.e., the set of all sufficient reasons) is of exponential size
%in the worst case.
%%For the classes of \cnf\ and \dnf\ formulas, it is well-known that an input instance can have exponentially many sufficient reasons.
%%For example, the monotone \cnf\ formula $F = \bigwedge_{i=1}^{\lfloor\frac{n}{2}\rfloor} (x_{2i-1} \vee x_{2i})$ has $2^{\lfloor\frac{n}{2}\rfloor}$.
%%prime implicants, each of them being implied by $\vec x = (1,1,\cdots,1)$. Surprisingly, 
%Indeed, even for the restricted class of decision trees of 
%logarithmic depth, an input instance can have exponentially many sufficient reasons:
%
%\begin{proposition}\label{prop:nbDT}
%%    Let $\dt^k_{n}$ be the class of decision trees of depth $k \geq 1$ over $n = 2^k - 1$ variables. Then, t
%There is a decision tree $T$ of depth $k \geq 1$ over $n = 2^k - 1$ variables
% such that for any $\vec x \in \{0,1\}^n$, the number of sufficient reasons for $\vec x$ given $T$ is at least $\lfloor \frac{3}{2}^{\frac{n + 1}{2}} \rfloor$. 
%\end{proposition}

%\paragraph{Probabilistic Reasons.} 

\subsection{Probable Reasons}

\pierre{Voir si on garde tout ce qui suit.}

A natural way to circumvent the computational barrier of finding minimal reasons is to rely on a probabilistic notion of prime implicant explanations,
as suggested in \cite{WALDCHEN2020}. This leads to generalize the notion of sufficient reasons, instead of refining it.
Basically, the idea of ``probable`'' prime implicants stems from the fact that standard, ``logical'' prime implicants 
are often too rigid for high dimensional, and possibly noisy, classification tasks. Thus, by forgetting few models of the classifier $f$, 
probable prime implicants may provide much shorter explanations. Formally, let $\PP_{\vec z}[f(\vec z)]$ be the probability 
that an assignment $\vec z$, drawn at random according to the uniform distribution over $\{0,1\}^n$, is a model of $f$, i.e.
\begin{align*}
\PP_{\vec z}[f(\vec z)] = \frac{\size{\vec z \in \{0,1\}^n: f(\vec z) = 1}}{\size{\vec z \in \{0,1\}^n}}
\end{align*}
Now, let $\PP_{\vec z}[f(\vec z) \mid t \subseteq t_{\vec z}]$ be the conditional probability that a random assignment $\vec z$ is a model of $f$, 
given that $\vec z$ is an extension of $t$:

\begin{align*}
\PP_{\vec z}[f(\vec z) \mid t \subseteq t_{\vec z}] = \frac{\size{\vec z \in \{0,1\}^n: f(\vec z) = 1 \mbox{ and } t \subseteq t_{\vec z}}}{\size{\vec z \in \{0,1\}^n: t \subseteq t_{\vec z}}}
\end{align*}


For a confidence parameter $\delta \in [0, 1]$, a term $t$ is called a $\delta$-\emph{probable implicant} of $f$ 
if $\PP_{\vec z}[f(\vec z) \mid t \subseteq t_{\vec z}] \geq \delta$, 
that is, the proportion of extensions of $t$ that are models of $f$ is at least $\delta$. If $t$ is a $\delta$-probable implicant of $f$ and no proper subset of $t$ 
is a $\delta$-probable implicant of $f$, then $t$ is called a $\delta$-\emph{probable prime implicant} of $f$.

\begin{definition}[$\delta$-Probable Reason] 
    Let $f \in \mathcal F_n$ and $\vec x \in \{0,1\}^n$ such that $f(\vec x) = 1$.
    A \emph{$\delta$-probable reason} for $\vec x$ given $f$ is a $\delta$-probable prime implicant $t$ of $f$ such that $t \subseteq t_{\vec x}$.
\end{definition}

\begin{example}
    For our running example, we can observe that $x_2 \land x_4$ is not a sufficient reason for $\vec x$ given $F$, but it is
    still a $75\%$-probable reason for $\vec x$ (given $F$).
\end{example}
    
%Clearly enough, considering $\delta$-probable reasons can also be a way to get rid of incomprehensible characteristics in sufficient reasons
%(even if there is no guarantee that incomprehensible characteristics are systematically removed).

% \begin{definition}[Approximate Implicant]
% Let $\delta \in [0, 1]$. A term $t$ is a $\delta$-\emph{approximate implicant} of a Boolean function $f \in \mathcal F_n$ if and only if
% $f \mid t$ has a number of models (over its set of variables) that is $\geq \delta \times 2^{|\mathit{Var}(f \mid t)|} $.
% \end{definition}
% Thus, any term is a $0$-approximate implicant of $f$ and the implicants $t$ of $f$ are precisely the 
% $1$-approximate implicants of $\Sigma$.
% On this basis, we can easily define a notion of approximate reason:
%
%\begin{definition}[prime approximate implicant]
%Let $\delta \in [0, 1]$. A term $\gamma$ is a \emph{prime} $\delta$-\emph{approximate implicant} of a Boolean function $\Sigma$ if and only if
%$\gamma$ is a $\delta$-approximate implicant of $\Sigma$, and $\gamma$ deprived of any of its literal $\ell$ is not a $\delta$-approximate 
%implicant of $\Sigma$.
%\end{definition}
% \begin{definition}[Approximate Reason]
% Let $\delta \in [0, 1]$. 
% \begin{itemize}
% \item A term $t$ is a \emph{prime} $\delta$-\emph{approximate implicant} of a Boolean function $f \in \mathcal F_n$ if and only if
% $t$ is a $\delta$-approximate implicant of $f$, and $t$ deprived of any of its literal $\ell$ is not a $\delta$-approximate 
% implicant of $f$.
% \item A term $t$ is an $\delta$-\emph{approximate reason} for an instance $\vec{x} \in \{0,1\}^n$  given a Boolean function $f \in \mathcal F_n$ if and only if
% $t$ is a prime $\delta$-approximate implicant of $f$ such that $\vec{x} \models t$ holds.
% \end{itemize}
% \end{definition}
% Note that focusing on $\delta$-\emph{approximate reasons} instead of sufficient reasons not only is a way to get shorter (thus more intelligible)
% explanations, but also to get rid of mandatory features that can be unintelligible by the explainee.

Interestingly, the problem of computing a $\delta$-probable reason for an instance given a decision tree
can be shown as tractable \cite{ref-our-paper-submitted-to-ijcai21}.
%This can be done by slightly modifying the greedy algorithm for sufficient reasons. Namely, at each iteration $i \in [n]$, 
%instead of testing whether the current term $t$, deprived from the literal $l_i$, is an implicant of $T$, we check whether $t \setminus \{l_i\}$ is a $\delta$-probable implicant 
%of $T$. Using the fact that conditioning and model counting operations can be done in linear time for decision trees \cite{Koricheetal13}, the inequality 
%$\PP_{\vec z}[f(\vec z) \mid t \subseteq t_{\vec z}] \geq \delta$ can be checked in linear time. %To sum up:
%
%\begin{proposition}\label{prop:probabilisticreasonDT}
%Let $T \in \dt_n$ and $\vec{x} \in \{0,1\}^n$ such that $T (\vec{x}) = 1$.
%Then, finding a $\delta$-probable reason for $\vec x$ given $T$ can be done in $O(n\size{T})$ time.
%\end{proposition}
%
Unfortunately, this result cannot be extended to the case of random forests:

\begin{proposition}\label{prop:probabilisticreasonRF}
    Let $F \in \rf_{n,m}$ and $\vec x \in \{0,1\}^n$ such that $F(\vec x) = 1$.
%    Unless {\sf P = NP}, there is no polynomial-time algorithm for computing a $\delta$-probable reason for $\vec x$ given $F$.
 Computing a $\delta$-probable reason for $\vec x$ given $F$ is {\sf \#P}-hard.
\end{proposition}

%\color{blue}

That mentioned, the greedy algorithm for computing sufficient reasons as presented in Section \ref{sec:sufficient}
can be modified to compute $\delta$-probable reasons. What needs to be updated only is the implicant test 
$t \models F$ that is used. When dealing with sufficient reasons, an exact test is required. When dealing with
$\delta$-probable reasons, it is acceptable that a small proportion of the models of $t$ (smaller than $\delta$) 
are not models of $F$. Deciding it boils down to counting the number of models of $t \wedge \neg F$. Since $F$ can be turned
in polynomial time into a \cnf\ formula provided that additional variables are considered (cf. Proposition \ref{prop:implicanttestRF}),
one can thus take advantage of a {\it projected model counter} (see e.g., \cite{LagniezMarquis19} to decide whether a 
given term $t$ is or not a $\delta$-probable implicant of a random forest $F$.

%\color{black}

%Nonetheless, the greedy algorithm presented in Section \ref{sec:sufficient} can be easily modified for computing a $\delta$-probable reason for $\vec x$ given 
%a random forest $F$. The key issue is here to be able to determine whether or not a given term $t$ (obtained by removing literals from $t_{\vec x})$ is 
%a $\delta$-probable implicant of $F$. To do so, it is enough to count the number of models over $X_n$ of $\exists \{y_1, \ldots, y_m\}. (C_{\mathrm{hard}} \wedge t)$
%(where $C_{\mathrm{hard}}$ is the hard constraint as given in Proposition \ref{prop:minimaloptim}) and then to check whether or not this number is at least equal 
%to $\delta \cdot 2^n$. Noticeably, the computation of the number of models over $X_n$ of $\exists \{y_1, \ldots, y_m\}. (C_{\mathrm{hard}} \wedge t)$ amounts to
%solving an instance of the \emph{projected model counting problem} \cite{Klebanovetal13}, for which some pieces of software exist \cite{Azizetal15,LagniezMarquis19}.
%
%To conclude with probable reasons, note that if one wants to put things together and compute a minimal $\delta$-probable reason, i.e., $\delta$-probable reason of minimal size, 
%the problem to be tackled would be even harder from the computational side (computing a minimal $\delta$-probable reason is an ${\sf NP^{PP}}$-hard problem
%in the general case, see Theorem 2.4 in \cite{WALDCHEN2020}). 


% From this proposition, we can easily design a polynomial-time greedy algorithm for deriving a $\delta$-approximate reason 
% for any instance $\vec{x}$ given a decision tree $T$ (this algorithm is very close to the one used for deriving a sufficient reason, which
% is sketched above).
%sketched in the proof of Proposition \ref{prop:onesufficientRF}).


==> conclusion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}\label{conclusion}

\pierre{A compléter plus tard.}

%\pierre{TBC. Recall the main contributions and give some perspectives. Computing all the reasons.} 

%It is acknowledged that intelligibility is among the research questions pertaining to XAI that have not been 
%explored in depth, and that it should receive more attention  \cite{doshivelez2017rigorous,GuidottiMRTGP19}. Our work contributes 
%to fill the gap, with a study of the intelligibility question for decision trees and random forests.
%We have shown that it is possible to derive in polynomial time a sufficient reason for a given instance $\vec x$ when the classifier is a random forest.
%We have argued that such a reason cannot be guaranteed as intelligible in the general case because it may contain too many 
%characteristics.
%To deal with this issue, we have focused on a refinement and on a generalization of the notion of sufficient reasons, 
%namely the minimal reasons and the probable reasons, respectively.
%We have identified the complexity of computing such reasons for a given instance when the classifier is a decision tree or a random forest, 
%and we have described  exact or approximate algorithms for deriving them.  Though the derivation of a sufficient reason for any given instance
%is tractable for both ML models, decision trees can be considered as more interpretable than random forests in the sense that deriving
% (or approximating) minimal or probable reasons looks more amenable for the former than for the latter.
%We have also presented
%empirical results for illustrating the gain in intelligibility they may offer and 
%the performances of the algorithms for computing them. 

%It is acknowledged that intelligibility is among the research questions pertaining to XAI that have not been 
%explored in depth, and that it should receive more attention  \cite{doshivelez2017rigorous,GuidottiMRTGP19}. Our work contributes 
%to fill the gap, with a study of the intelligibility question for decision trees and random forests.
%Though a sufficient reason for any prediction can be computed efficiently given such classifiers,
%we have argued that it cannot be guaranteed as intelligible in the general case because it may contain too many 
%characteristics and/or characteristics that are not comprehensible by the explainee.
%To deal with this issue, we have presented several refinements / generalizations of the notion of sufficient reasons.
%We have identified the complexity of computing such reasons for a given instance when the classifier is a decision tree or a random forest, 
%and we have described  exact or approximate algorithms for deriving them.  We have also presented
%empirical results for illustrating the gain in intelligibility they may offer and 
%the performances of the algorithms for computing them. 




==> experiments.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}\label{experiments}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\color{blue}

We have performed a number of experiments in order (i) to evaluate the gain in intelligibility 
that results from focusing on the sizes of the direct sufficient, minimal and $\delta$-probable reasons, relatively to the size of the instances, and (ii) 
to evaluate the practical performance of the algorithms for computing them.

\subsection{Empirical setting}

The empirical protocol was as follows. 
We have considered 90 datasets, which are standard benchmarks from the well-known repositories Kaggle\footnote{\url{www.kaggle.com}}, OpenML\footnote{\url{www.openml.org}}, 
and UCI\footnote{\url{archive.ics.uci.edu/ml/}}. Due to space constraints, the complete list of benchmarks used is reported as a supplementary material, 
together with additional information about the decision trees and the sizes of the different reasons that have been computed.
Several datasets considered in our experiments include a large number of instances with a large number of features.     
Because some datasets are suited to the multi-label classification task, we used the standard ``one versus all'' policy to deal with them: 
all the classes but the target one are considered as the complementary class of the target.
Categorical features have been treated as arbitrary numbers (the scale is nominal). 
As to numeric features, no data preprocessing has taken place: these features have been binarized on-the-fly 
by the decision tree learning algorithm that has been used.

% further details about the corresponding trees and 
%the computations of the various notions of reasons considered in the paper.
% Some of the datasets gather large numbers of instances, based on large numbers of features (see Table \ref{tab:results} for details).
%For example, the dataset "Dexter" contains $2600$ instances, based on $20 000$ features, and the dataset "p53 mutant" contains $16772$ instances based on $5409$ attributes.
% Some of them concern more than one class (and its complementary class).  To deal with such datasets, a ``one versus al'' policy 
% has been considered:  all the classes but the target one are considered as the complementary class of the target.
% Categorical features are treated as arbitrary numbers (the scale is nominal). As to numeric features, no preprocessing has taken place,
% all numeric features have been binarized on-the-fly by the algorithm used for generating decision trees.

%For every benchmark $b$, a $10$-fold cross validation process has been achieved. 
%Namely, a set of $10$ decision trees $T_b$ have been computed and evaluated
%from the labelled instances of $b$, partitioned into $10$ parts. 
%One part was used as the test set and the remaining $9$ parts as the training set for generating
%a decision tree. This tree is thus in 1-to-1 correspondence with the test set chosen within the whole dataset $b$.
%The classification performance for $b$ was measured as the mean accuracy obtained over the $10$ decision trees
%generated from $b$. 

For the random forest learner, we have used the ??? algorithm \pierre{à compléter et ajouter une réf} 
and more specifically its implementation provided by the \textrm{Scikit-Learn}\footnote{scikit-learn.org/stable/index.html} 
library. %\cite{scikit-learn} --> Ce serait bien de les citer, mais par équité ce serait bien aussi de citer les auteurs de Pysat :-)
%\footnote{\url{scikit-learn.org/stable/modules/generated/sklearn.tree.DecisionTreeClassifier.html}} 
All hyper-parameters of the learning algorithm have been set to their default value.
%Notably, decision trees have been learned using the Gini criterion, and without any maximal depth or any other manual limitation. 

% using a Python  3.7.9 program based on the Scikit-Learn library, release 0.23.2\footnote{\url{https://scikit-learn.org/stable/}}. 
% The "DecisionTreeClassifier" class of this library (\url{https://scikit-learn.org/stable/modules/generated/sklearn.tree.DecisionTreeClassifier.html}) 
% has been used, each parameter being set to its default value. Especially, the Gini criterion was considered to build the decision trees.
% No maximal depth or any other manual limitation was preset. 

For each benchmark $b$, each random forest $F$, and each instance $\vec x$ of the corresponding test set, 
we computed the direct reason for $\vec x$ given $F$, a sufficient reason for $\vec x$ given $F$, 
a minimal reason for $\vec x$ given $F$, and $\delta$-probable reasons for $\vec x$ given $F$ for several values of 
$\delta$ ($95\%$, $90\%$, $75\%$). 

For computing sufficient (resp. minimal reasons), we used \pierre{ ... à compléter}
%the Pysat\footnote{\url{https://pysathq.github.io/}} library, which provides the implementation of the RC2 \textsc{Partial MaxSAT} solver.
%This solver was run using the parameters corresponding to the ``Glucose'' setting.
For each instance in a dataset and each type of reason, we computed the mean size of the reason 
(given as a number of binary features), together with the corresponding standard deviation.
In our experiments, we have also measured the runtimes required to compute any reason.
All the experiments have been conducted on a computer equipped with 
Intel(R) Core(TM) i9-9900 CPU @ 3.10 GHz  and 64 GiB of memory. 
%The kernel used was CentOS 7, Linux version 3.10.0-514.16.1.el7.x86\_64. 
%The compiler used was gcc version 5.3.1.
%Hyperthreading was disabled, and no cache share between cores was allowed.
%A time-out (TO) of 1h and a memory-out (MO) of 7.6 GiB has been considered for each instance. 

%For each benchmark $b$, all the elements of the dataset have been considered as instances $\vec x$.
%For every $\vec x$, the corresponding direct reason $p_{\vec x}^{T_b}$ given $T_b$ has been computed. We have also
%computed a sufficient reason for $\vec x$ given $T_b$ (starting the greedy algorithm on $p_{\vec x}^{T_b}$), and
%a minimal reason for $\vec x$ given $T_b$. Finally, for several values of $\delta$ ($95\%$, $90\%$, and $75\%$)\pierre{Vérifier} {\color{magenta} Steve : Tout me semble correcte, en revanche cela est un peu redondant avec la fin de mon paragraphe, il faudra sans doute fusionner les 2 explications}, we have
%computed a $\delta$-probable reason for $\vec x$ given $T_b$ (starting the greedy algorithm on the direct reason / the minimal
%reason \pierre{Vérifier} for $\vec x$ given $T_b$ that were computed previously). For every benchmark $b$, we have made some statistics about the sizes of 
%the reasons that have been computed when $\vec x$ varies in the dataset, and the computation times required to derive such reasons.

%For each benchmark, we took advantage of the Scikit-Learn to generate a decision tree \pierre{give more details, how many instances have been used, add references}.
%Then we picked up at random following a uniform distribution a set of instances $\vec x$ from the dataset such that this set contains 10\%
%of the total number of instances of the search space. For each instance $\vec x$, we have computed a corresponding reason for each notion of reason 
%(here, direct reasons, sufficient reasons, minimal reasons, and $\delta$-probable reasons) and we have measured its size. Figure \ref{???} 
%synthesizes using box plots the distribution of the sizes of the reasons for several benchmarks.
%
%If significant, one can also use scatter plots for some benchmarks (each dot corresponds to an $\vec x$, the size of its direct reason (for instance) is 
%represented on the $x$-axis and the size of its minimal reason (for instance) is represented on the $y$-axis).
%Is there a difference when focusing on instances that are misclassified by the decision tree?
%
%Discuss the obtained results.
%
%Figure \ref{???} presents using box plots the distribution of the computation times needed to extract a minimal reason from a direct reason
%for several benchmarks. For all the other notions of reasons, the computation times appear as negligible \pierre{Give more details.} 
%Discuss the results and the feasibility of the approach from the practical side.

%
%
%\begin{figure*}
% \includegraphics[width=0.5\textwidth]{farm-ads.png}
% \hfill
% \includegraphics[width=0.5\textwidth]{ad-data.png}
%  \begin{minipage}{0.5\textwidth}\centering Farm-ads\end{minipage}
%  \hfill\begin{minipage}{0.5\textwidth}\centering Ad-data\end{minipage}
% \caption{\label{fig:scatter}Comparison, for Farm-ads and Ad-data, between direct and sufficient reason (resp. 75\%-probable reason). Each dot represents
% an instance, the $x$-axis gives the size of its direct reason and the $y$-axis gives the size of the sufficient reason (resp. 75\%-probable reason) computed from the
% direct reason.}
% \end{figure*}

\subsection{Results}

\pierre{A compléter quand on les aura : l'idée est de lancer le même type d'expés que pour le papier soumis à IJCAI'21}

%\color{black}

==> introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\color{blue}

Explaining the predictions achieved by machine learning (ML) models is a topic of tremendous importance for
a couple of years. A popular ML model consists of random forests \cite{DBLP:journals/pami/Ho98,DBLP:journals/ml/Breiman96b,DBLP:journals/ml/Breiman01},
which are mainly collections of decision trees  \cite{DBLP:books/wa/BreimanFOS84,DBLP:journals/ml/Quinlan86}. Random forests are typically more accurate
classifiers than decision trees, especially because they are more robust to the noise that may pertain the data from which the classifier is generated.
However, random forests are usually considered as less interpretable than decision trees. Indeed, given a decision tree $T$ and an instance $\vec x$ to be classified,
one can derive in polynomial time a ``direct reason'' $p_{\vec x}^T$ explaining the classification done by $T$ on $\vec x$. The direct reason $p_{\vec x}^T$
for $\vec x$ given $T$ is a subset the characteristics of $\vec x$ such that every instance $\vec x'$ sharing this subset of characteristics would be classified
by $T$ in the same way as $\vec x$. The direct reason $p_{\vec x}^T$ corresponds to the (unique) path of $T$ that is compatible with $\vec x$.

On the other hand, a number of notions of reasons for Boolean classification, suited to the local explanation issue, but not specific to a particular ML model (as decision trees)
have been pointed out recently on the literature. Thus, a {\em sufficient reason} \cite{DarwicheHirth20} (also known as prime implicant explanations \cite{ShihCD18}) for an instance $\vec x$ given a class described by a Boolean function $f$ is a subset $t$ of the characteristics of $\vec x$ that is minimal w.r.t. set inclusion and such that any instance $\vec x'$ sharing this set $t$ of characteristics is classified by $f$ as $\vec x$ is. Thus, when $f(\vec x) = 1$, $t$ is a sufficient reason for $\vec x$ given $f$ if and only if $t$ is a prime implicant of $f$ such that $\vec x$ implies $t$, and when $f(\vec x) = 0$, $t$ is a sufficient reason for $\vec x$ given $f$ if and only if $t$ is a prime implicant of $\neg f$ such that $\vec x$ implies $t$.
A {\em minimal reason} for $\vec x$ given $f$  \cite{ref-our-paper-submitted-to-ijcai21} is a sufficient reason for $\vec x$ given $f$ containing a minimal number of characteristics. A concept of {\em $\delta$-probable reason} for $\vec x$ given $f$  (where $\delta \in [0, 1]$) has also been pointed out \cite{ref-our-paper-submitted-to-ijcai21} in order to relax the entailment condition
of the implicant test and deal with noisy data.

Comparing random forests to decision trees, there is a clear gap as to the local explanation issue. On the one hand, there is no notion of direct reason suited
to random forests. On the other hand,  though algorithms for computing sufficient, minimal or $\delta$-probable reasons for decision tree classifiers exist  \cite{ref-our-paper-submitted-to-ijcai21},
\pierre{Voir si on garde les $\delta$-probable reasons} there are no such algorithms for random forests. In order to fill the gap, we introduce a concept of direct reason for the case of decision trees and we show that such a reason for an instance $\vec x$ given a random forest $F$ can be computed in time linear in the size of $F$ and the size of $\vec x$. We also 
present and evaluate algorithms for computing sufficient, minimal or $\delta$-probable reasons for random forests. Sufficient (resp. minimal reasons)
can be characterized in terms of MUSes, alias minimal unsatisfiable subsets of \cnf\ formulae (resp. MUSes of minimal size). Such characterizations 
are valuable since they allow for leveraging the many {\sc SAT}-based algorithms for computing MUSes in order to derive sufficient or minimal reasons.
We present complexity results showing that using an algorithm for computing a MUS in order to derive a sufficient reason is not using a sledgehammer
to crack a nut: testing whether a term is a sufficient reason is precisely as hard as testing whether a subset of clauses is a MUS of a \cnf\ formula.
We also explain how $\delta$-probable reasons can be computed using a projected model counter.
Finally, we present the results of an empirical study based on random forests generated from many datasets.
Explanations have been computed for the instances belonging to those datasets, under the form of direct, sufficient, minimal, or $\delta$-probable reasons.
The results obtained from the experimentations show from a practical side the intelligibility of the explanations that have been derived
(in terms of their number of features compared to the number of features in the instances) and the efficiency of the algorithms
to generate them.\pierre{A affiner quand on aura les résultats expérimentaux.}

The rest of the paper is organized as follows. 
Section \ref{preliminaries} is about decision trees and random forests.
The various notions of reasons considered in the paper as well as algorithms for computing them, are presented in Section \ref{sec:sufficient}.
%Minimal reasons and probable reasons are presented in Section \ref{beyond}.
Some mepirical results are given and analyzed in Section \ref{experiments}.
Finally, Section \ref{conclusion} concludes the paper. Proofs are provided as
supplementary material.

%\color{black}

%Explaining a decision is the process used to make a human being understand why the decision has been made. 
%This is a significant issue, especially when decisions are generated automatically by AI systems, 
%including classifiers and other machine learning (ML) models.  
%In the context of classification, the decision to be explained is the concept (class) that is predicted
%from the input instance.
%
%Of course, deriving explanations calls for dedicated technologies. Given the importance
%of the issue, there has been a growing body of work on explainable and robust AI (XAI) for the past couple of years 
%(see for instance \cite{DBLP:conf/aaai/IgnatievNM19,DBLP:conf/nips/BunelTTKM18,DBLP:journals/corr/abs-1805-09938,DBLP:conf/sat/ShihDC19,GuidottiMRTGP19,DBLP:journals/ai/Miller19,Molnar19}). %DBLP:journals/jossw/MolnarCB18,
%\pierre{This list must be updated.}
%
%Among ML models used for the classification purpose are \emph{decision trees} \cite{DBLP:books/wa/BreimanFOS84,DBLP:journals/ml/Quinlan86}, which are popular models because they are usually considered as highly interpretable. Furthermore, decision trees are key components of more sophisticated (actually, more accurate) 
%%but often viewed as less interpretable) 
%ML models, namely random forests, which are mainly collections of decision trees \cite{DBLP:journals/pami/Ho98,DBLP:journals/ml/Breiman96b,DBLP:journals/ml/Breiman01}. 
%%Furthermore, there are many work centered on distilling better ML models (in terms of prediction) into decision trees so as to benefit from their interpretability \pierre{Add references}.
%
%%But why are decision trees usually considered as \emph{interpretable models}? Basically, this is because of the \emph{local explanation facility} they support: from any instance $\vec x$ to be classified and a decision tree used as a classifier, one can easily get, together with the class that is predicted for the instance, a subset $p$ of its characteristics such that every instance $\vec x'$ sharing this subset $p$ of characteristics would be classified in the same way as $\vec x$. The set $p$ corresponds to the (unique) path of the decision tree that is compatible with $\vec x$. The set $p$ can be computed efficiently (that is, in time linear in the size of the input). Furthermore, $p$ can be considered as a better explanation of the prediction made for $\vec x$ than $\vec x$ itself because $p$ contains (in general) less characteristics than $\vec x$.
%
%%Pushing this idea a step further and abstracting it away from decision trees, 
%Though there is no consensus on what explaining precisely means for human beings (see for instance \cite{DBLP:journals/corr/abs-1802-00682,DBLP:journals/ai/Miller19,DBLP:conf/ijcai/0002C20}), when it comes to the explanation of classification of instances, the notion of \emph{sufficient reasons} \cite{DarwicheHirth20} (also known as prime implicant explanations \cite{ShihCD18}) appears as a valuable candidate. 
%A sufficient reason for an instance $\vec x$ given a class described by a Boolean function $f$ such that $f(\vec x) = 1$ is a subset $t$ of the 
%characteristics of $\vec x$ that is minimal w.r.t. set inclusion and such that any instance $\vec x'$ sharing this set $t$ of characteristics is classified by $f$ as $\vec x$ is.
%Due to the minimality condition w.r.t. set inclusion, sufficient reasons do not contain any characteristic that would be redundant 
%for the explanation task at hand, in the sense that removing any feature from a sufficient reason $t$ for $\vec x$ given $f$
%would lead to question the covering question (i.e., the fact that any instance $\vec x'$ sharing this set $t$ of characteristics is classified 
%by $f$ as $\vec x$ is). The significance of sufficient reasons comes from Occam's razor (roughly stating that the best explanations 
%are the simpler ones). The simplicity criterion is quite fundamental: it must be kept in mind that explaining is a social process \cite{DBLP:journals/ai/Miller19},
%where explainees are human beings, that have (inherently) \emph{cognitive limitations}. Thus, in his seminal paper (that marked the beginning of cognitive psychology as a field) \cite{Miller56}, psychologist George Miller introduced the idea of people “chunking” items (i.e., grouping them together as a unit) and argued that
%due to human memory limitations, the size of chunks is limited to 7, plus or minus 2. Ever since then, many experiments in cognitive science has
%confirmed this limitation. Restricting explanations to contain only few characteristics thus appears as an important requirement for ensuring that they are intelligible.
%
%Albeit there is no formal definition of what an interpretable ML model should be \cite{DBLP:journals/cacm/Lipton18}, decision trees are usually considered 
%as interpretable. There are two main reasons for it: their decomposability property (each node in a decision tree has some meaning, and the principles used for generating
%a decision tree can be justified), and the \emph{local explanation facility} they provide: from any instance $\vec x$ to be classified and a decision tree 
%$T$ used as a classifier, one can easily get, together with the class that is predicted for the instance, a subset $p$ of its characteristics such that every instance $\vec x'$ sharing this subset $p$ of characteristics would be classified in the same way as $\vec x$. The set $p$ corresponds to the (unique) path of the decision tree that is compatible with $\vec x$, and it can be computed efficiently (that is, in time linear in the size of the input).
%Though the explanations $p$ that can be generated from input instances $\vec x$ given a decision tree $T$ contain typically far less characteristics than $\vec x$ itself,
%some recent work has shown that 
%%from the theory side 
%$p$ may contain arbitrarily many more characteristics than a sufficient reason for $\vec x$ given $T$ \cite{DBLP:journals/corr/abs-2010-11034}). 
%From the practical side, experiments reported in the same paper have pointed out that the number of extra characteristics contained in ``direct reasons'' 
%$p$ can be significantly larger than the size of sufficient reasons. Fortunately, one can take advantage of a greedy algorithm to eliminate efficiently 
%from $p$ any redundant characteristic, and this results in a polynomial-time algorithm for computing one sufficient reason for $\vec x$ given $T$. 
%
%In this perspective, two research questions naturally emerge:
%\begin{itemize}
%\item Is it possible to derive in polynomial time a sufficient reason for a given instance $\vec x$ when the classifier does not 
%reduce to a single decision tree $T$, but is a random forest $F$?
%\item Whatever the classifier (here, a decision tree or a random forest), what if the sufficient reason that has been computed 
%contains too many characteristics for being considered as intelligible by the explainee?
%\end{itemize}
%
%These are the main research questions considered in the paper. 
%As to the first question, we show that the greedy algorithm 
%for deriving a sufficient reason for a given instance given a decision tree 
%can be easily lifted to the case of a random forest $F$, without questioning its tractability.
%As to the second question, we consider a notion of  \emph{minimal reasons} that focuses on sufficient reasons of minimal size, and  a notion of  
%\emph{probable reasons}, that  generalizes the one of sufficient reasons by (roughly speaking) neglecting some instances $\vec x'$
%provided that there are only few of them. In both cases, we identify the
%complexity of computing a reason for a given instance when the classifier is a decision tree or a random forest, 
%and we describe exact or approximate algorithms for deriving such reasons.  
%We focus here on Boolean features \pierre{To be commented, is it without any loss of generality because other features can
%be binarized if needed? References are expected here.}
%Finally, the paper reports empirical results illustrating, from the practical side, the 
%gain in intelligibility that is obtained via the refinements of the notion of sufficient reasons
%that are considered and the performances of the algorithms that are pointed out. 
%
%The rest of the paper is organized as follows. % \textcolor{blue}{TBC. }
%Some background about decision trees and random forests is given in Section \ref{preliminaries}.
%The greedy algorithm for computing sufficient reasons given a random forest is pointed out in Section \ref{sec:sufficient}.
%Minimal reasons and probable reasons are presented in Section \ref{beyond}.
%Experimental results are described in Section \ref{experiments}.
%Finally, Section \ref{conclusion} concludes the paper. Proofs are provided as
%supplementary material.

%Furthermore, as shown in the following, 
%this algorithm can be easily lifted to the case of a random forest $F$ without questioning its tractability. Thanks to it, deriving explanations of the classifications
%of instances (under the form of sufficient reasons) appear as amenable for random forests. This is a first contribution of the paper.
%
%Does it mean that the game is over, and the question of explaining predictions from decision trees or, more generally, for random forests is fully addressed? 
%Not really, because sufficient reasons cannot be guaranteed to be intelligible enough. Especially, what if the sufficient reason that has been computed 
%contains too many characteristics for being considered as intelligible by the explainee?
%\begin{enumerate}
%\item What if the sufficient reason that has been computed contains some features that are not understandable by the explainee, or contain
%characteristics that are considered as unexpected, while neglecting characteristics that are considered as expected by the explainee?
%\item What if the sufficient reason that has been computed contains too many characteristics for being considered as intelligible by the explainee? 
%\end{enumerate}

%These are the main research questions considered in the paper. 
%Our objective is to contribute to address them.
%To this purpose, we present some refinements of the notion of sufficient reasons.  
%Thus, the notions of \emph{comprehensible reasons} and \emph{inclusion-preferred reasons} are introduced as a contribution to the first issue, and
%notions of \emph{minimal reasons} (and more generally of \emph{minimal-weight reasons}) as a contribution to the second issue. 
%We also present a notion of  \emph{probabilistic reasons}, that  generalizes sufficient reasons and
%prove useful for both issues. In both cases, we identify the
%complexity of computing a reason for a given instance when the classifier is a decision tree or a random forest, and we describe exact or approximate algorithms 
%for deriving such reasons.  
%We focus here on Boolean features \pierre{To be commented, is it without any loss of generality because other features can
%be binarized if needed? References are expected here.}
%Finally, the paper reports empirical results illustrating, from the practical side, the 
%gain in intelligibility that is obtained via the refinements / extensions of the notion of sufficient reasons
%that are introduced and the performances of the algorithms that are pointed out. 

%The rest of the paper is organized as follows. % \textcolor{blue}{TBC. }
%Some background about decision trees and random forests is given in Section \ref{preliminaries}.
%The greedy algorithm for computing sufficient reasons given a random forest is defined in Section \ref{sec:sufficient}.
%The main definitions and results from the theory side are presented in Section \ref{beyond}.
%Experimental results are described in Section \ref{experiments}.
%Finally, Section \ref{conclusion} concludes the paper. Proofs are provided as
%supplementary material.


==> preliminaries.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Decision Trees and Random Forests}\label{preliminaries}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For an integer $n$, let $[n] = \{1,\cdots,n\}$.
By $\mathcal F_n$ we denote the class of all Boolean functions from $\{0,1\}^n$ to $\{0,1\}$,
and  we use $X_n  = \{x_1, \cdots, x_n\}$ to denote the set of input Boolean variables. 
Any assignment $\vec x \in \{0,1\}^n$ is called an \emph{instance}. If $f(\vec x) = 1$ 
for some $f \in \mathcal F_n$, then $\vec x$ is called a \emph{model} of $f$.
We refer to $f$ as a propositional formula when it is described using the Boolean connectives $\land$ (conjunction), $\lor$ (disjunction) and 
$\neg$ (negation), together with the Boolean constants $1$ (true) and $0$ (false). 
As usual, a \emph{literal} $l_i$ is a variable $x_i$ or its negation $\neg x_i$, also denoted $\overline x_i$.
A \emph{term} (or \emph{monomial}) $t$ is a conjunction of literals, and a \emph{clause} $c$ is a disjunction of literals. 
%For a clause $c$ and an instance $\vec x$, $c[\vec x]$ denotes the subclause of $c$ consisting of all literals $\ell$ of $c$
%such that $\ell(\vec x) = 1$. --> Super ambigu comme notation, on peut confondre cela avec la valeur de la fonction booleenne c sur x.
A \emph{\dnf\ formula} is a disjunction of terms and a \emph{\cnf\ formula} 
is a conjunction of clauses. The set of variables occurring in a formula $f$ is denoted $\Var{f}$.

With these basic notions in hand, we shall focus on the following representation class of Boolean functions.

\begin{definition}[Decision Tree \& Random Forest] 
    \leavevmode
    \begin{itemize}
    \item A \emph{decision tree} on $X_n$ is a binary tree $T$, each of whose internal nodes is labeled with one of
    $n$ input variables, and whose leaves are labeled $0$ or $1$. Every variable is supposed (wlog) to occur at most once on any root-to-leaf path (read-once property).  
    The value $T(\vec x) \in \{0,1\}$ of $T$ on an input instance $\vec x$ is given by the label of the
    leaf reached from the root as follows: at each node go to the left or right child depending on whether the input value of the corresponding variable is $0$ or $1$, 
    respectively.  
    \item  A \emph{random forest} on $X_n$ is a multiset $F = \{T_1, \cdots, T_m\}$ of decision trees on $X_n$.\footnote{We can assume without any
    loss of generality that $m$ is odd. Indeed, if $m$ is even, it is enough to consider $F \cup \{1\}$ instead of $F$ since those two random forests are equivalent.}
    The value $F(\vec x) \in \{0,1\}$ of $F$ on an instance $\vec x\in \{0,1\}^n$ is obtained via a majority vote over the decision trees, that is,
        \begin{align*}
        F(\vec x) = 
            \begin{cases}
                1 & \mbox{ if } \frac{1}{m}\sum_{i=1}^m T(\vec x)  > \frac{1}{2} \\
                0 & \mbox{ otherwise.}
            \end{cases}
        \end{align*}
    \end{itemize}
\end{definition}

The size of a random forest $F = \{T_1,\cdots,T_m\}$ is given by $\size{F} = \sum_{i=1}^m \size{T_i}$,
where $\size{T_i}$ is the number of nodes occurring in $T_i$. The class of decision trees on 
$X_n$ is denoted $\dt_n$, and the class of random forests with at most $m$ decision trees (with $m \geq 1$)
over $\dt_n$ is denoted $\rf_{n,m}$. $\rf$ is the union of all $\rf_{n,m}$ for integers $n, m$.

%Note that any Boolean function in $\mathcal F_n$ can be represented by a decision tree
%in $\dt_n$ with $2^n$ leaves and depth of $n + 1$. 
%Since the sample complexity of $\dt_n$ is exponential in $n$, most 
%theoretical results about decision trees focus on restricted subclasses, such as the class  
%$\dt^k_n$ of decision trees on $X_n$ of depth $k$. By extension, we use $\rf^k_{m,n}$ 
%to denote the class of random forests with at most $m$ decision trees over $\smash{\dt^k_{n}}$.

Clearly enough, any Boolean function in $\mathcal F_n$ can be represented by a decision tree
in $\dt_n$, thus by a random forest in $\rf_{n,m}$ whatever $m$.  

It is well-known that computing the negation of a given decision tree $T \in \dt_n$ can be done in linear time
(just replace every $1$-leaf in $T$ by a $0$-leaf, and vice-versa).
%, and that the disjunction of two decision trees
%$T_1, T_2 \in dt_n$ can be achieved in time $\size{T_1}\cdot \size{T_2}$ (replace every $0$-leaf in $T_1$
%by a copy of $T_2$, then replace in the resulting tree every decision  node $N$ over variable $x_i$ by its left child (resp. right child) 
%whenever it is a descendant of another decision  node $M$ over variable $x_i$ obtained by following the left arc (resp. right arc)
%outgoing from $M$ - this is for ensuring the read-once property of decision trees), see \cite{Koricheetal13} for details.
%Due to De Morgan's laws, this shows that a decision tree representing the conjunction of two decision trees
%$T_1, T_2 \in dt_n$ can also be computed in time polynomial in the input size.
Interestingly, negating a random forest can also be achieved in polynomial time:

\begin{proposition}\label{prop:transfoRF}~
There exists a polynomial-time algorithm that computes a random forest $F' \in \rf_{n,m}$ that is equivalent to
the negation of a given random forest $F \in \rf_{n,m}$.
\end{proposition}

It is also well-known that any decision tree $T \in \dt_n$ can be transformed in linear time into an equivalent disjunction of terms, denoted $\dnf(T)$,
where each term coincides with a $1$-path, i.e., a path from the root to a leaf labeled with $1$. $T$ can also be transformed in linear time into 
a conjunction of clauses, denoted $\cnf(T)$, where each clause is the negation of the term describing a $0$-path, i.e., a path from the root to a leaf labeled with $0$.
However, the converse does not hold. Indeed, $\dt_n$ is a subset of the language \fbdd, the free binary decision diagrams over $X_n$ \cite{GergovMeinel94}, 
and it is known that \fbdd\ is not at least as succinct as \cnf\ or \dnf\ (see Proposition 3.1 in \cite{DarwicheMarquis02}). This means that there exist families
of \cnf\ (or \dnf) formulae $\varphi_n$ over a set of $n$ variables such that any \fbdd\ representation of $\varphi_n$ has a size superpolynomial in $\size{\varphi_n}$.
As a consequence, there cannot be any polynomial-time algorithm for turning a \cnf\ (or \dnf) formula into an equivalent \fbdd\ representation.

When switching from decision trees to random forests, the connections to \cnf\ and \dnf\ flip. To be more precise:

\begin{proposition}\label{prop:CNF2RF} Any  \cnf\ or \dnf\ formula can be converted in linear time into an equivalent random forest, but
neither \cnf\ nor \dnf\ is at least as succinct as the language \rf\ of random forests.
\end{proposition}


% When several decision trees are considered at the same time, one gets a a random forest:
% \begin{definition}[Random Forest] 
%     The value $F(\vec x) \in \{0,1\}$ of $F$ on an instance $\vec x\in \{0,1\}^n$ is obtained via a majority vote over the decision trees, that is,
%     \begin{align*}
%         F(\vec x) = 
%         \begin{cases}
%             1 & \mbox{ if } \frac{1}{m}\sum_{i=1}^m T(\vec x)  > \frac{1}{2} \\
%             0 & \mbox{ otherwise.}
%         \end{cases}
%     \end{align*}% The size of a random forest $F = \{T_1, \cdots, T_m\}$ is given by $\size{F} = \sum_{i=1}^m \size{T}$.
%and $\rf^k_{n,m}$, 
% we denote the classes of random forests with at most $m$ decision trees in $\dt_n$. % and $\dt^k_n$, respectively.
% \end{definition}


==> rushes.tex <==

% %Although minimal sufficient reasons look too computationally demanding, minimal majoritary reasons 
% %appear as an interesting compromise: their size and the computational effort required to generate them
% %are typically smaller than those obtained for sufficient reasons.

% % and much smaller than those associated with LIME explanations). 
% % Majoritary reasons and minimal majoritary reasons are specific to ensemble methods. 
% % Minimal sufficient reasons, i.e., sufficient reasons of minimal size, are more general (as sufficient reasons, they make sense for any Boolean classifier). 
% % We compare all those explanations w.r.t. both the complexity dimension and the size dimension.  
% % We also add to the comparison the heuristic explanations obtained as the minimal sufficient reasons for the instances given the corresponding 
% % linear models generated using LIME \cite{Lime16} (note that there is no guarantee that such ``LIME explanations'' are abductive ones).
% % More in detail, we present some complexity results pertaining to the generation of abductive explanations for the various families of explanations that are considered.
% % Thus, direct reasons and majoritary reasons can be derived in time polynomial in the size of the input (the instance and the random forest used to classify it).
% % Contrastingly, the identification of minimal majoritary reasons is {\sf NP}-complete, and the identification of minimal sufficient reasons is $\Sigma_2^p$-complete.
% % We also provide algorithms for deriving explanations from random forest classifiers, which open the way for an empirical comparison. 
% % The experiments made on standard benchmarks show the existence of a trade-off between the complexity of generating abductive explanations and 
% % the size of the explanations that are derived. Minimal sufficient reasons look too computationally demanding. 
% % Minimal majoritary reasons appear as an interesting compromise (their size and the computational effort required to generate them
% % are typically smaller than those obtained for sufficient reasons, and much smaller than those associated with LIME explanations). 

% %fred : j'hesite à mettre ce paragraphe qui fait très "bateau".
% %Computational complexity it is not the unique dimension that must be taken into account when evaluating the quality of an abductive explanation. 
% %The size of the explanation that is generated matters as well, since explanations containing hundreds of features can hardly be considered as intelligible. Though sufficient reasons are irreducible explanations, an instance can be shown to have exponentially many sufficient reasons when the classifier is a random forest (indeed, it is already the case for decision tree classifiers).
% %Even if a ``quite short'' sufficient reason exists, there is no guarantee that the one returned by the MUS algorithm mentioned above is short.


% % Explaining the predictions achieved by machine learning (ML) models is a topic of tremendous importance for
% % a couple of years. A popular ML model consists of random forests 
% % QA1\cite{DBLP:journals/pami/Ho98,DBLP:journals/ml/Breiman96b,DBLP:journals/ml/Breiman01},
% % which are mainly collections of decision trees  \cite{DBLP:books/wa/BreimanFOS84,DBLP:journals/ml/Quinlan86}. Random forests are typically more accurate
% % classifiers than decision trees, especially because they are more robust to the noise that may pertain t
% % he data from which the classifier is generated.
% % However, random forests are usually considered as less interpretable than decision trees. 
% % Indeed, the generation of a \emph{(local) abductive explanation}, i.e., a
% % subsets of features of the instance at hand that is enough to explain the prediction made on it by the classifier, is computationally easy when the classifier is a
% % decision tree. To be more precise, given a decision tree $T$ and an instance $\vec x$ to be classified, one can derive in polynomial time the ``direct reason'' %$t_{\vec x}^T$ 
% % explaining the classification done by $T$ on $\vec x$. 
% %The direct reason $t_{\vec x}^T$
% %for $\vec x$ given $T$ is a subset the characteristics of $\vec x$ such that every instance $\vec x'$ sharing this subset of characteristics would be classified
% %by $T$ in the same way as $\vec x$. 
% %This direct reason $t_{\vec x}^T$ 
% % This direct reason corresponds to the (unique) path of $T$ that is compatible with $\vec x$. It may contain characteristics that are
% % useless for explaining the prediction made by $T$ on $\vec x$. Nevertheless, a {\em sufficient reason} \cite{DarwicheHirth20} 
% % that does not suffer from this drawback can be extracted from the direct reason
% %$t_{\vec x}^T$ via 
% % using a polynomial-time algorithm when the classifier is a decision tree. Thus, a sufficient reason for an instance $\vec x$ given a Boolean classifier $f$ 
% % (which can be a decision tree, a random forest or any other Boolean classifier) is a subset $t$ of the characteristics of $\vec x$ that is minimal w.r.t. set inclusion  such that any instance $\vec x'$ sharing this set $t$ of characteristics is classified by $f$ as $\vec x$ is. 
% %Thus, when $f(\vec x) = 1$, $t$ is a sufficient reason for $\vec x$ given $f$ if and only if $t$ is a prime implicant of $f$ such that $\vec x$ implies $t$, and when $f(\vec x) = 0$, $t$ is a sufficient reason for $\vec x$ given $f$ if and only if $t$ is a prime implicant of $\neg f$ such that $\vec x$ implies $t$. 
% % Stated otherwise, sufficient reasons are abductive explanations $t$ for $\vec x$ given $f$ such that $t$ is irreducible (removing any characteristics from $t$ would question the fact that $t$ explains the way $\vec x$ is classified by $f$).
% % Contrastingly, no notion of ``direct reason'' has been considered so far for random forests. Furthermore, the computation of a sufficient reason for an input instance given a random forest
% % has been considered only in the very recent past \cite{joao-ijcai21}, where the problem has been shown intractable (identifying a sufficient reason being {\sf DP}-complete).\footnote{We assume the reader acquainted with basics of complexity theory (see e.g., \cite{Papadimitriou94} otherwise).} 
% % Despite this intractability statement, the empirical results reported in \cite{joao-ijcai21} show that a MUS-based algorithm for computing a sufficient reason proves quite efficient in practice.

% % Fred: Non, on ne fait generalement pas une décomposition de l'article dans NIPS.
% % The rest of the paper is organized as follows. 
% % Section \ref{preliminaries} gives some preliminaries and present some results about decision trees and random forests.
% % The various notions of reasons considered in the paper, some complexity results about their generation as well as algorithms for computing them, are presented in Section \ref{sec:explanations}.
% % Some empirical results about the time needed to compute abductive explanations and about the sizes of those explanations
% % are given and analyzed in Section \ref{experiments}.
% % Finally, Section \ref{conclusion} concludes the paper. 
% % Proofs and additional empirical results are provided as supplementary material.

% %i.e., a path from the root to a leaf labeled with $1$. $T$ can also be transformed in linear time into 
% %a conjunction of clauses, denoted $\cnf(T)$, where each clause is the negation of the term describing a $0$-path, i.e., a path from the root to a leaf labeled with $0$.
% % However, the converse does not hold. Indeed, $\dt_n$ is a subset of the language \fbdd, the free binary decision diagrams over $X_n$ \cite{GergovMeinel94}, 
% % and it is known that \fbdd\ is not at least as succinct as \cnf\ or \dnf\ (see Proposition 3.1 in \cite{DarwicheMarquis02}). This means that there exist families
% % of \cnf\ (or \dnf) formulae $\varphi_n$ over a set of $n$ variables such that any \fbdd\ representation of $\varphi_n$ has a size superpolynomial in $\size{\varphi_n}$.
% % As a consequence, there cannot be any polynomial-time algorithm for turning a \cnf\ (or \dnf) formula into an equivalent \fbdd\ representation.

% % Clearly enough, any Boolean function in $\mathcal F_n$ can be represented by a decision tree
% % in $\dt_n$, thus by a random forest in $\rf_{n,m}$ whatever $m$.  
% %It is well-known that computing the negation of a given decision tree $T \in \dt_n$ can be done in linear time
% %(just replace every $1$-leaf in $T$ by a $0$-leaf, and vice-versa).
% %It is also well-known that any decision tree $T \in \dt_n$ can be transformed in linear time into an equivalent disjunction of terms, denoted $\dnf(T)$,
% %where each term coincides with a $1$-path, i.e., a path from the root to a leaf labeled with $1$. $T$ can also be transformed in linear time into 
% %a conjunction of clauses, denoted $\cnf(T)$, where each clause is the negation of the term describing a $0$-path, i.e., a path from the root to a leaf labeled with $0$.
% %
% %, and that the disjunction of two decision trees
% %$T_1, T_2 \in dt_n$ can be achieved in time $\size{T_1}\cdot \size{T_2}$ (replace every $0$-leaf in $T_1$
% %by a copy of $T_2$, then replace in the resulting tree every decision  node $N$ over variable $x_i$ by its left child (resp. right child) 
% %whenever it is a descendant of another decision  node $M$ over variable $x_i$ obtained by following the left arc (resp. right arc)
% %outgoing from $M$ - this is for ensuring the read-once property of decision trees), see \cite{Koricheetal13} for details.
% %Due to De Morgan's laws, this shows that a decision tree representing the conjunction of two decision trees
% %$T_1, T_2 \in dt_n$ can also be computed in time polynomial in the input size.
% % Interestingly, negating a random forest can also be achieved in polynomial time:

% % \begin{definition}[Decision Tree \& Random Forest] 
% %     \leavevmode
% %     \begin{itemize}
% %     \item A \emph{decision tree} on $X_n$ is a binary tree $T$, each of whose internal nodes is labeled with one of
% %     $n$ input variables, and whose leaves are labeled $0$ or $1$. Every variable is supposed (wlog) to occur at most once on any root-to-leaf path (read-once property).  
% %     The value $T(\vec x) \in \{0,1\}$ of $T$ on an input instance $\vec x$ is given by the label of the
% %     leaf reached from the root as follows: at each node go to the left or right child depending on whether the input value of the corresponding variable is $0$ or $1$, 
% %     respectively.  %The \emph{direct reason} for $\vec x$ given $T$ is the term, denoted $t_{\vec x}^T$, corresponding to the unique root-to-leaf path of $T$ that is compatible with $\vec x$. 
% %     \item  A \emph{random forest} on $X_n$ is an ensemble-based classifier $F = \{T_1, \cdots, T_m\}$ on $X_n$ where each $T_i$ ($i \in [m]$) is a decision tree on $X_n$.
% % %    \item  A \emph{random forest} on $X_n$ is a multiset $F = \{T_1, \cdots, T_m\}$ of decision trees on $X_n$.\footnote{We can assume without any
% % %    loss of generality that $m$ is odd. Indeed, if $m$ is even, it is enough to consider $F \cup \{1\}$ instead of $F$ since those two random forests are equivalent.}
% % %    The value $F(\vec x) \in \{0,1\}$ of $F$ on an instance $\vec x\in \{0,1\}^n$ is obtained via a majority vote over the decision trees, that is,
% % %        \begin{align*}
% % %        F(\vec x) = 
% % %            \begin{cases}
% % %                1 & \mbox{ if } \frac{1}{m}\sum_{i=1}^m T(\vec x)  > \frac{1}{2} \\
% % %                0 & \mbox{ otherwise.}
% % %            \end{cases}
% % %        \end{align*}
% %     \end{itemize}
% % \end{definition}


% %\color{blue}
% %fred: c'est complètement faux. 
% % \begin{definition}[Ensemble-Based Classifier]
% % An \emph{ensemble-based classifier} on $X_n$ is a multiset $E = \{f_1,$ $\cdots,$ $f_m\}$ of Boolean functions from 
% % $\mathcal F_n$.\footnote{We can assume without any loss of generality that $m$ is odd. Indeed, if $m$ is even, it is enough to consider $E \cup \{1\}$ instead of $E$ since those two classifiers are equivalent.} The value $E(\vec x) \in \{0,1\}$ of $E$ on an instance $\vec x\in \{0,1\}^n$ is obtained via a majority vote over the Boolean functions of $E$, that is,
% %         \begin{align*}
% %         E(\vec x) = 
% %             \begin{cases}
% %                 1 & \mbox{ if } \frac{1}{m}\sum_{i=1}^m f(\vec x)  > \frac{1}{2} \\
% %                 0 & \mbox{ otherwise.}
% %             \end{cases}
% %         \end{align*}
% % \end{definition}
% %\color{black}


% %Note that any Boolean function in $\mathcal F_n$ can be represented by a decision tree
% %in $\dt_n$ with $2^n$ leaves and depth of $n + 1$. 
% %Since the sample complexity of $\dt_n$ is exponential in $n$, most 
% %theoretical results about decision trees focus on restricted subclasses, such as the class  
% %$\dt^k_n$ of decision trees on $X_n$ of depth $k$. By extension, we use $\rf^k_{m,n}$ 
% %to denote the class of random forests with at most $m$ decision trees over $\smash{\dt^k_{n}}$.


% % When several decision trees are considered at the same time, one gets a a random forest:
% % \begin{definition}[Random Forest] 
% %     The value $F(\vec x) \in \{0,1\}$ of $F$ on an instance $\vec x\in \{0,1\}^n$ is obtained via a majority vote over the decision trees, that is,
% %     \begin{align*}
% %         F(\vec x) = 
% %         \begin{cases}
% %             1 & \mbox{ if } \frac{1}{m}\sum_{i=1}^m T(\vec x)  > \frac{1}{2} \\
% %             0 & \mbox{ otherwise.}
% %         \end{cases}
% %     \end{align*}% The size of a random forest $F = \{T_1, \cdots, T_m\}$ is given by $\size{F} = \sum_{i=1}^m \size{T}$.
% %and $\rf^k_{n,m}$, 
% % we denote the classes of random forests with at most $m$ decision trees in $\dt_n$. % and $\dt^k_n$, respectively.
% % \end{definition}

% %\input{sufficient}


% % % and such that $t$ is an implicant of $f$ if $f(\vec x)$

% % % such that $\vec x \models t$, 
% % % $t \models f$ if $f(\vec x) = 1$ and $t \models \neg f$ if $f(\vec x) = 0$.
 


% % % Suppose we are given a Boolean classifier $f \in \mathcal F_n$ together with an input instance $\vec x \in\{0,1\}^n$.
% % % The key focus of this study is to explain \emph{why} $f$ classifies $\vec x$ as positive or negative. %, when $f$ is a decision tree or a random forest. 
% % % %The \emph{reasons} for explaining the prediction made by $f$ on $\vec x$ typically take the form of a conjunction of literals
% % % This calls for a notion of abductive explanation:

% % % \begin{definition}[Abductive Explanation]
% % % Let $f \in \mathcal F_n$ be a Boolean classifier and let $\vec x \in \{0, 1\}^n$ be an instance.
% % % An {\em abductive explanation}\footnote{Unlike \cite{DBLP:conf/aaai/IgnatievNM19}, we do not require those explanations to be minimal w.r.t. set inclusion, in order to keep the concept 
% % % distinct (and actually more general) then the one of sufficient reasons.} $t$ for $\vec x$ given $f$ is a conjunction of literals such that $\vec x \models t$, 
% % % $t \models f$ if $f(\vec x) = 1$ and $t \models \neg f$ if $f(\vec x) = 0$.
% % % \end{definition}

% % An abductive explanation $t$ for $\vec x$ given $f$ always exists given that $t = t_{\vec x}$ is such a (trivial) explanation.

% % We mention in passing that we could have focused without loss of generality  
% % on the case $f(\vec x) = 1$ in the definition above (and in the forthcoming definitions), assuming that $f$ is given as a random forest.
% % Indeed (i) a reason why  $f(\vec x) = 0$ is precisely the same as a reason why $- f(\vec x) = 1$, and (ii) as shown by Proposition \ref{prop:transfoRF},
% % any representation $F \in  \rf_{n,m}$ of $f$ can be transformed in linear time into a representation $\neg F \in \rf_{n,m}$ 
% % of $-f$. 
% %Nevertheless, in the following, we consider most of the time both cases of positive and of negative instances for the sake of clarity.

% %Indeed, if $F = \{T_1,\cdots,T_m\}$ then $F' = \{\neg T_1,\cdots, \neg T_m\}$, where $\neg T_i$ is the decision 
% %obtained from $T_i$ by replacing the label of each leaf with its complement (see e.g. \cite{Koricheetal13}).

% %\color{blue}

% % \begin{definition}[Minimal Sufficient Reason] 
% % Let $f \in \mathcal F_n$ and $\vec x \in \{0,1\}^n$. % such that $f(\vec x) = 1$.
% % A \emph{minimal sufficient reason} for 
% % $\vec x$ given $f$ is a sufficient reason for $\vec x$ given $f$ that is of minimal size.\footnote{Minimal sufficient reasons should not to be confused with \emph{minimum-cardinality explanations}  \cite{ShihCD18}, where the minimality condition bears on the features set to $1$ in the input instance.}
% % \end{definition}


% %Given Proposition \ref{prop:sufficient reason-MUS-RF}, 


% % %As a by-product of Proposition \ref{prop:complexityminimalMUS}, 
% % Note that leveraging an algorithm for computing a minimal MUS in order to
% % compute a minimal sufficient reason looks as a reasonable approach because both problems have the same complexity 
% % (deciding whether there exists a MUS $I$ of $S$ given $H$ that contains at most $k$ literals also is $\Sigma_2^p$-complete, 
% % see \cite{DBLP:conf/cp/IgnatievPLM15,DBLP:journals/ai/Liberatore05}).
% % However, this high complexity (second level of the polynomial hierarchy) is an important obstacle for making the concept of minimal sufficient reason
% % practical enough for random forests (empirical results reported in Section \ref{experiments} will provide some evidence for this).\pierre{A ne pas oublier !}

% %Due to the primality condition, for every abductive explanation $t$ for $\vec x$ given $f$, there exists a sufficient reason $t'$ for $\vec x$ given $f$
% %such that $t' \models t$.

% % It is easy to show that the direct reason $t_{\vec x}^F$ for $\vec x$ given $F$ may contain arbitrarily many more features 
% % than a sufficient reason for $\vec x$ given $F$. Indeed, it has been shown recently that this is the case for decision trees \cite{DBLP:journals/corr/abs-2010-11034},
% % and the direct reason for an instance $\vec x$ given a random forest that contains a single tree $T$ coincides with the direct reason for $\vec x$ given $T$.
% % A similar result can be obtained for majoritary reasons:

% % \begin{proposition} \label{prop:majoritary}
% % Let $F = \{T_1, \ldots, T_m\}$ be a random forest of  $\rf_{n, m}$ and $\vec x \in \{0,1\}^n$ such that $F(\vec x) = 1$. Unless $m < 3$,
% % it can be the case that every majoritary reason for $\vec x$ given $F$ contains arbitrarily many more features 
% % than any sufficient reason for $\vec x$ given $F$.
% % \end{proposition}

% Actually, the notion of sufficient reason for $\vec x$ given a random forest appears as more tricky than the one for the case of decision trees. 
% The greedy algorithm sketched above for computing sufficient reasons in the case of decision trees can still be used
% for computing sufficient reasons given a random forest, but it must be based on an updated implicant test. Indeed, if 
% $t$ an implicant of at least $\lfloor \frac{m}{2} \rfloor +1$ decision trees of $F$, then $t$ clearly is an implicant of $F$, but the
% converse does not hold (otherwise, the notions of majoritary reasons and of sufficient reasons would coincide, but this is
% not the case as a by-product of Proposition \ref{prop:majoritary}).
% %
% %Especially, though the implicant test for decision trees can be achieved efficiently, it is more complex in the case of random forests.
% %
% %Especially, in the case of a random 
% %forest $F$, focusing on the sufficient reasons for $\vec x$ given the trees of $F$ is not enough to characterize  the sufficient 
% %reasons for $\vec x$ given $F$. 
% %More than that, focusing on the implicants $t$ of a majority of decision trees $T \in F$ such that $\vec x \models t$ holds 
% %is not enough. As a matter of illustration, consider $F = \{T_1, T_2, 1\}$ where $T_1$ is a decision tree equivalent to $x_1 \wedge x_2$
% %and $T_2$ is a decision tree equivalent to $x_1 \wedge \overline{x}_2$. $F$ is equivalent to $x_1$. The (unique) sufficient reason for 
% %$\vec x = (1, 1)$ is $x_1$, but $x_1$ neither is an implicant of $t_1$ nor is an implicant of $T_2$.
% %
% %Nevertheless, two observations are worth being made: (1) the use of this greedy algorithm for generating sufficient reasons is not
% %specific to decision trees, but it works for any Boolean classifier $f \in \mathcal F_n$ (possibly not in polynomial time,
% %depending on the nature of $f$), and (2) the key test in this construction is the implicant one
% %(testing whether a term is an implicant of $T$) that is iterated. This test is where the computational complexity of
% %the greedy algorithm lies. For decision trees $T$, this test is quite simple and can be achieved in polynomial time (a consistent term $t$ is an implicant of 
% %a decision tree $T$ when $t$ intersects every clause of $\cnf(T)$), and as a consequence, the greedy algorithm
% %for deriving a sufficient reason for $\vec x$ given $T$ also runs in polynomial time. 
% %


% %   \begin{align*}
% %        C_{\mathrm{soft}} &= \{\overline x_i  : x_i \in t_{\vec x}\} \cup \{x_i  : \overline x_i \in t_{\vec x}\} \\
% %        C_{\mathrm{hard}} &= \{(\overline y_i \vee c_{\mid \vec x}) : i \in [m], c \in \cnf(T_i) \} \cup \cnf(\sum_{i = 1}^m y_i > \frac{m}{2})
% %    \end{align*}


% Seemingly, one can hardly do better and design a polynomial-time algorithm for the implicant test, since this would imply that {\sf P = NP}: 

% %Interestingly, the {\sc SAT}-based implicant test for random forests given by Proposition \ref{prop:implicanttestRF} is only ``mildly hard''. 
% Going one step further, the sufficient reasons for an instance $\vec x$ given a random forest $F$ can be characterized in terms of
% MUS (minimal unsatisfiable subsets) \cite{joao-ijcai21}. 
% %Given a set of clauses $S$ that is satisfiable and a set of clauses $H$ such that $S \cup H$ is unsatisfiable,
% %a MUS of $S$ given $H$ is a subset $I$ of clauses of $S$ such that $I \cup H$ is unsatisfiable, but for every clause $c \in I$, $(I \setminus \{c\}) \cup H$ 
% %is satisfiable. $H$ is a set of so-called hard clauses and $S$ (disjoint from $H$) contains the so-called soft clauses.  
% %A MUS is thus a subset $I$ of $S$ which is jointly unsatisfiable
% %with $H$ but becomes satisfiable with $H$ as soon as a single clause of $I$ is removed from $I$.
% %Note that one can assume without any loss of generality that 
% %$S = \{c_i : i \in \{1, \ldots, k\}\}$ is a set of literals (indeed, one can always replace $H$ by a \cnf\ formula $H' = H \cup \{\overline{y_i} \vee c_i : i \in \{1, \ldots, k\}\}$ 
% %and $S$ by $S' = \{y_1, \ldots, y_k\}$ in such a way that $I$ is a MUS of $S$ given $H$ if and only if 
% %$M' = \{y_i : c_i \in I\}$ is a MUS of $S'$ given $H'$).
% %
% %\begin{proposition} \label{prop:sufficient reason-MUS-RF}
% %    Let $F \in \rf_{n, m}$ and $\vec x \in \{0,1\}^n$ such that $F(\vec x) = 1$. 
% %    Let $t$ be a term over $X_n$ such that $t \subseteq t_{\vec x}$. $t$ is a sufficient reason for $\vec x$ given $F$ if and only if
% %    $t$ is a MUS of $S= \{\ell : \ell \in t_{\vec x}\}$ given $H$, the \cnf\ formula given in Proposition \ref{prop:implicanttestRF}.
% %\end{proposition}
% %
% %Note that a MUS-based characterization of the sufficient reasons for an instance $\vec x$ given a random forest $F$ has been pointed out very recently \cite{joao-ijcai21}.
% %However, the approach used in \cite{joao-ijcai21} is quite different from ours regarding the binary features appearing in the explanations. Indeed, in \cite{joao-ijcai21},
% %the dataset is first binarized using the direct encoding (alias the one-hot encoding) technique \cite{}\pierre{Ajouter une réf}, then
% %a random forest is learned from this dataset; contrastingly, in our approach, the binary features are those occurring in the decision trees
% %of the random forest that has been learned (the dataset is not binarized first, but on-the-fly). Note that binarizing the features at start precludes
% %from considering numeric features in \cite{joao-ijcai21} (only binary and categorical features can be dealt with), while our approach
% %does not suffer from this limitation.\pierre{A vérifier absolument !}
% %%et sans doute en dire plus. Il faudrait surtout voir si expérimentalement les sufficient reasons calculées par Joao restent bien en général de tailles plus grandes que nos minimal majoritary reasons.}
% %The characterization result given by Proposition \ref{prop:sufficient reason-MUS-RF} 
% %Whatever the approach used,  a MUS-based characterization of the sufficient reasons is valuable from a computational perspective 
% This characterization is useful because many {\sc SAT}-based algorithms  for computing a MUS (or even all MUSes) of a \cnf\ formula have been pointed out for the past decade
% \cite{DBLP:conf/sat/AudemardLS13,DBLP:journals/constraints/LiffitonPMM16,DBLP:journals/ai/Marques-SilvaJM17} \pierre{Voir si ces réfs sont OK.} 
% One can take advantage of them for computing sufficient reasons (and this is what we did in our experiments). 
% %Note that when the objective is to compute a single sufficient reason for $\vec x$ given $F$ using an algorithm for computing a MUS, we could consider $S = \{\ell : \ell \in t_{\vec x}^F\}$ 
% %or $S$ as the set of literals of any majoritary reason for $\vec x$ given $F$ instead of considering $S = \{\ell : \ell \in t_{\vec x}\}$.

% %This time again, one can hardly expect to do much better and design a polynomial-time algorithm for computing a sufficient reason.
% %%Indeed, as a consequence of Proposition \ref{prop:complexitysufficientreasonRF}, 
% %Thus, the tractability result about the generation of a sufficient reason 
% %for  $\vec x$ given a decision tree cannot be lifted to the more general case of a random forest, unless {\sf P = NP}.
% %Indeed, deciding whether a term $t$ is a sufficient reason for  an instance $\vec x$ given a random forest $F$ is {\sf DP}-complete \cite{joao-ijcai21}.
% %
% %%\begin{proposition} \label{prop:complexitysufficientreasonRF}
% %%    Let $F \in \rf_{n, m}$ and $\vec x \in \{0,1\}^n$ such that $F(\vec x) = 1$. 
% %%    Deciding whether a term $t$ is a sufficient reason for  $\vec x$ given $F$ is {\sf DP}-complete.
% %%    %in {\sf DP} and is both {\sf NP}-hard and {\sf coNP}-hard.
% %%\end{proposition}
% %
% %%As a by-product of Proposition \ref{prop:complexitysufficientreasonRF}, 
% %This complexity result shows that using a MUS-based approach for computing 
% %a sufficient reason does not look as using a sledgehammer to crack a nut:
% %deciding whether $I$ is a MUS of $S$ given $H$ also is {\sf DP}-complete.
% %Furthermore, though the MUS-based algorithms to compute a sufficient reason do not run in polynomial time in the worst case, 
% %the tremendous progress in {\sc SAT} solving achieved for 
% %the past two decades, makes them quite practical in many cases  (see Section \ref{experiments}).


% or $\neg F$ if $F(\vec x) = 0$. If so, remove $\ell$ from $t$ and proceed to the next literal.
% Once all literals in $t_{\vec{x}}$ have been examined, the final term $t$ is by construction an implicant of a strict majority 
%  such that
% removing any literal from it would lead to a term that is not any longer an implicant of $T$ (resp. $\neg T$). Thus, $t$

% This algorithm elaborates on the greedy algorithm for computing a sufficient reason
% for $\vec x$ given a decision tree. Indeed, for decision trees $T \in \dt_n$, it is already known that deriving a sufficient reason for $\vec x$ given $T$ 
% such that $T(\vec x) = 1$ (resp. $T(\vec x) = 0$) can be done in polynomial time (see e.g., \cite{DBLP:journals/corr/abs-2010-11034}).
% %,ref-our-paper-submitted-to-ijcai21}). 
% The computation is as follows: start with $t = t_{\vec x}$, and iterate over the literals $\ell$ of
% $t$ by checking whether $t$ deprived of $\ell$ is an implicant of $T$ (resp. $\neg T$), which boils down to check whether $t$ intersects every clause of $\cnf(T)$ 
% (resp. $\cnf(\neg T)$ and can be done in linear time. If so, remove $\ell$ from $t$ and proceed to the next literal.
% Once all literals in $t_{\vec{x}}$ have been examined, the final term $t$ is by construction an implicant of $T$ such that
% removing any literal from it would lead to a term that is not any longer an implicant of $T$ (resp. $\neg T$). Thus, $t$
% is a prime implicant of $T$ (resp. $\neg T$) containing only literals from $\vec{x}$, alias a sufficient reason for $\vec x$ given $T$.

% In the case of majoritary reasons, the implicant test must be updated in such a way that $\ell$ is removed if and on if
% $t$ deprived of $\ell$ is an implicant of a strict majority of trees in $F$ if $F(\vec x) = 1$ and a strict majority of trees in $\neg F$ if $F(\vec x) = 0$. 
% Of course, the greedy algorithm based on the updated 
% implicant test runs in time polynomial in the size of the input. Note also that instead of starting it with $t = t_{\vec x}$, the greedy algorithm
% can be run with $t = t_{\vec x}^F$ or, more generally, with any term $t$ such that $t \subseteq t_{\vec x}$ and 
% $t$ an implicant of at least $\lfloor \frac{m}{2} \rfloor +1$ decision trees of $F$ if $F(\vec x) = 1$ (resp. of $\neg F$ if $F(\vec x) = 0$). 
% Doing so, the correctness of the greedy algorithm
% would not be questioned (and its efficiency could possibly be improved via less implicant tests).

%\color{black}
%More generally, the notion of majoritary reason can be defined for any ensemble-based classifier:
%such that $F(\vec x) = 1$ (resp. $F(\vec x) = 0$).
%A {\em majoritary reason} for $\vec x$ given $F$ is a term $t$ over $X_n$ such that $t \subseteq t_{\vec x}$, $t$ is an implicant of at least $\lfloor \frac{m}{2} \rfloor +1$
%decision trees $T_i$ (resp. $\neg T_i$) where $T_i \in F$, and for every $\ell \in t$, $t \setminus \{\ell\}$ does not satisfy this last condition.
%%\color{blue}
%\begin{definition}[Majoritary Reason]
%Let $E = \{f_1, \ldots, f_m\}$ be an ensemble-based classifier on $X_n$ and let $\vec x \in \{0, 1\}^n$ be an instance such that $E(\vec x) = 1$ (resp. $E(\vec x) = 0$).
%A {\em majoritary reason} for $\vec x$ given $E$ is a term $t$ over $X_n$ such that $t \subseteq t_{\vec x}$, $t$ is an implicant of at least $\lfloor \frac{m}{2} \rfloor +1$
%functions $f_i$ (resp. $-f_i$) where $f_i \in E$, and for every $\ell \in t$, $t \setminus \{\ell\}$ does not satisfy this last condition.
%\end{definition}
%%\color{black}

%When $F$ consists of a single decision tree $T$, the minimal majoritary reasons for $\vec x$ given $F$ coincide with the 
%minimal sufficient reasons for $\vec x$ given $T$, i.e., the sufficient reasons for $\vec x$ given $F$ that are of minimal size.
%However, computing a minimal sufficient reason for an instance given a decision tree is intractable in the general case:
%\pierre{C'est dans le papier DT mais le résultat est un peu différent  - appartenance à NP} 
%As a consequence, c


==> sufficient.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Reasons}\label{sec:sufficient}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Suppose we are given a Boolean classifier $f \in \mathcal F_n$ together with an input instance $\vec x \in\{0,1\}^n$.
The key focus of this study is to explain \emph{why} $f$ classifies $\vec x$ as positive, when $f$ is a decision tree or a random forest. 
The \emph{reasons} for explaining $f(\vec x) = 1$ typically take the form of a conjunction of literals which together justify the prediction 
made by $f$ on $\vec x$. 

We mention in passing that focusing on $f(\vec x) = 1$ is without any loss of generality for decision trees and random forests, 
since (i) a reason why  $f(\vec x) = 0$ is precisely the same as a reason why $- f(\vec x) = 1$, and (ii) as show by Proposition \ref{prop:transfoRF},
any representation $F \in  \rf_{n,m}$ of $f$ can be transformed in linear time into a representation $F' \in \rf_{n,m}$ 
of $-f$. 
%Indeed, if $F = \{T_1,\cdots,T_m\}$ then $F' = \{\neg T_1,\cdots, \neg T_m\}$, where $\neg T_i$ is the decision 
%obtained from $T_i$ by replacing the label of each leaf with its complement (see e.g. \cite{Koricheetal13}).

In the rest of the paper, we shall often treat assignments as terms, and terms as sets of literals. 
Given an assignment $\vec z \in \{0,1\}^n$, the corresponding term is defined as
\begin{align*}
t_{\vec z} = \bigwedge_{i=1}^n x_i^{z_i} \mbox{ where } x_i^0 = \overline x_i \mbox{ and } x_i^1 = x_i
\end{align*}
A term $t$ \emph{covers} an assignment $\vec z$ if $t \subseteq t_{\vec z}$. An \emph{implicant} of a Boolean function $f$
is a term that implies $f$, that is, a term $t$ such that $f(\vec z) = 1$ for every assignment $\vec z$ covered by $t$. A \emph{prime implicant}
of $f$ is an implicant $t$ of $f$ such that no proper subset of $t$ is an implicant of $f$. 

%\color{blue}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Direct Reasons}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Given a decision tree $T$, with every instance $\vec x$ such that $T(\vec x) = 1$ one can associate a term $p_{\vec x}^T$, called the direct reason
for $\vec x$ given $T$. $p_{\vec x}^T$ corresponds to the unique root-to-leaf path of $T$ that is compatible with $\vec x$. Thus, $p_{\vec x}^T$
is such that $\vec x \models p_{\vec x}^T$ and $p_{\vec x}^T \models T$.
Similarly, we can introduce a notion of direct reason $p_{\vec x}^F$ for $\vec x$ given a random forest $F = \{T_1, \ldots, T_m\}$: 

\begin{definition}[Direct Reason]
Let $F = \{T_1, \ldots, T_m\}$ be a random forest from $\rf$ and let $\vec x \in \{0, 1\}^n$ be an instance such that $F(\vec x) = 1$.
The {\em direct reason} $p_{\vec x}^F$ for $\vec x$ given $F$ is the conjunction of all the direct reasons $p_{\vec x}^{T_i}$ for those decision trees 
$T_i$ of $F$ such that $T_i (\vec x) = 1$.
Using symbols:
$$p_{\vec x}^F = \bigwedge_{T_i \in F : T_i(\vec x) = 1} p_{\vec x}^{T_i}.$$
\end{definition}

By construction, $p_{\vec x}^F$ is such that $\vec x \models p_{\vec x}^F$ and $p_{\vec x}^F \models F$.
Obviously, $p_{\vec x}^F$ can be computed in time polynomial in the size of $F$ and the size of $\vec x$.

\pierre{Cela vaudra le coût de calculer la taille de ces direct reasons en pratique via des expérimentations à base de random forests.}

\begin{figure}[t]
\centering
\scalebox{0.5}{
      \begin{tikzpicture}[scale=0.9] 
        \node[ellipse,draw](root) at (2,7){$x_4$};
        \node at (0.5,7){$T_1$};
        \node(n1) at (1,5){$0$};  
        \node[ellipse,draw](n2) at (3,5){$x_2$};
        \node(n21) at (2,3){$1$};          
        \node[ellipse,draw](n22) at (4,3){$x_3$};  
        \node(n221) at (3,1){$0$};  
        \node[ellipse,draw](n222) at (5,1){$x_1$};   
        \node(n2221) at (4,-1){$0$}; 
        \node(n2222) at (6,-1){$1$}; 
        \draw[densely dotted] (root) -- (n1);
        \draw(root) -- (n2);
        \draw[densely dotted] (n2) -- (n21);
        \draw(n2) -- (n22);    
        \draw[densely dotted] (n22) -- (n221);
        \draw(n22) -- (n222);  
        \draw[densely dotted] (n222) -- (n2221);
        \draw(n222) -- (n2222);
                
        \node[ellipse,draw](root2) at (9,7){$x_2$};
        \node at (7.5,7){$T_2$};
        \node[ellipse,draw](n2-1) at (8,5){$x_1$};  
        \node(n2-2) at (10,5){$1$};
        \node(n2-11) at (7,3){$0$};          
        \node[ellipse,draw](n2-12) at (9,3){$x_4$};  
        \node(n2-121) at (8,1){$0$};  
        \node(n2-122) at (10,1){$1$};   
        \draw[densely dotted] (root2) -- (n2-1);
        \draw(root2) -- (n2-2);
        \draw[densely dotted] (n2-1) -- (n2-11);
        \draw(n2-1) -- (n2-12);    
        \draw[densely dotted] (n2-12) -- (n2-121);
        \draw(n2-12) -- (n2-122);  
        
        \node[ellipse,draw](root3) at (16,7){$x_3$};
        \node at (14.5,7){$T_3$};
        \node[ellipse,draw](n3-1) at (14,5){$x_2$};  
        \node[ellipse,draw](n3-2) at (17,5){$x_2$};  
        \node[ellipse,draw](n3-11) at (13,3){$x_1$};
        \node[ellipse,draw](n3-12) at (15,3){$x_4$};   
        \node(n3-121) at (14.5,1){$0$};   
        \node[ellipse,draw](n3-122) at (16,1){$x_1$};  
        \node(n3-1221) at (15,-1){$0$};     
        \node(n3-1222) at (17,-1){$1$};          
        \node(n3-21) at (16.5,3){$0$};
        \node[ellipse,draw](n3-22) at (18,3){$x_4$};     
        \node(n3-111) at (12,1){$0$};  
        \node(n3-112) at (13.5,1){$1$}; 
        \node(n3-221) at (17.5,1){$0$};  
        \node(n3-222) at (19,1){$1$};           
        \draw[densely dotted] (root3) -- (n3-1);
        \draw(root3) -- (n3-2);
        \draw[densely dotted] (n3-1) -- (n3-11);
        \draw(n3-1) -- (n3-12);    
        \draw[densely dotted] (n3-2) -- (n3-21);
        \draw(n3-2) -- (n3-22); 
        \draw[densely dotted] (n3-11) -- (n3-111);
        \draw(n3-11) -- (n3-112);  
        \draw[densely dotted] (n3-22) -- (n3-221);
        \draw(n3-22) -- (n3-222);
        \draw[densely dotted] (n3-12) -- (n3-121);
        \draw(n3-12) -- (n3-122);
        \draw[densely dotted] (n3-122) -- (n3-1221);
        \draw(n3-122) -- (n3-1222);
      \end{tikzpicture}
 }
    \caption{A random forest $F = \{T_1, T_2, T_3\}$ for recognizing {\it Cattleya} orchids. The left (resp. right) child of any decision node labelled by $x_i$ corresponds to 
    the assignment of $x_i$ to $0$ (resp. $1$).\label{fig:orchids}}
    \end{figure}

\begin{example}\label{running-ex}
The random forest $F = \{T_1, T_2, T_3\}$ in Figure \ref{fig:orchids} separates {\it Cattleya} orchids from other orchids using the following features:
\begin{itemize}
\item $x_1$: ``has fragrant flowers'';
\item $x_2$: ``has one or two leaves'';
\item $x_3$: ``has large flowers'';
\item $x_4$: ``is sympodial'';
\item $x_5$: ``has white flowers''.
\end{itemize}
The instance $\vec x = (1, 1, 1, 1, 1)$ is recognized as a {\it Cattleya} orchid, since $F(\vec x) = 1$.
The direct reason for $\vec x$ given $F$ is $p_{\vec x}^F = x_1 \land x_2 \land x_3 \land x_4$. It is better than $\vec x$ itself
since it does not contain $x_5$, which turns out to be globally irrelevant ($x_5$ does not appear in any decision tree of $F$).
%The term $t = x_1 \land x_2 \land x_3 \land x_4$, corresponding to the unique root-to-leaf path that is compatible with $\vec x$,
%can be viewed as a ``direct reason'' for $\vec x$ given $T_1$. 
%Note that $t$ is an implicant of $F$ covering $\vec x$, but it is \emph{not} a sufficient reason.
%Indeed, $t$ can be further reduced to the conjunction $t' = x_2 \wedge x_3 \wedge x_4$, 
%which is a prime implicant of $F$ covering $\vec x$, and hence, a sufficient reason for $\vec x$ given $F$.
\end{example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proto-Sufficient Reasons}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Inspired by the way sufficient reasons can be computed when dealing with decision trees, one can introduce the following concept of proto-sufficient reason.
As the notion of direct reason defined above, proto-sufficient reasons do not concern every Boolean classifier but are specific to random forests.

\begin{definition}[Proto-Sufficient Reason]
Let $F = \{T_1, \ldots, T_m\}$ be a random forest from $\rf$ and let $\vec x \in \{0, 1\}^n$ be an instance such that $F(\vec x) = 1$.
A {\em proto-sufficient reason} for $\vec x$ given $F$ is a term $t$ over $X_n$ such that $t \subseteq t_{\vec x}$, $t$ an implicant of at least $\lfloor \frac{m}{2} \rfloor +1$
decision trees of $F$, and for every $\ell \in t$, $t \setminus \{\ell\}$ does not satisfy this last condition.
\end{definition}

\begin{example} For our running example, $\vec x$ has three proto-sufficient reasons given $F$: $x_1 \land x_2 \land x_4$, $x_1 \land x_3 \land x_4$, and 
$x_2 \land x_3 \land x_4$. Those reasons are better than $p_{\vec x}^F$ in the sense that they are shorter than the direct reason.
\end{example}

What makes proto-sufficient reasons valuable is that there exists a polynomial-time algorithm for computing a proto-sufficient reason for 
an instance $\vec x$ given a random forest $F$. This algorithm elaborates on the greedy algorithm for computing a sufficient reason
for $\vec x$ given a decision tree. Indeed, for decision trees $T \in \dt_n$, it is already known that deriving a sufficient reason for $\vec x$ given $T$ 
such that $T(\vec x) = 1$ can be done in polynomial time (see e.g., \cite{DBLP:journals/corr/abs-2010-11034,ref-our-paper-submitted-to-ijcai21}). The computation
is as follows: start with $t = t_{\vec x}$, and iterate over the literals $\ell$ of
$t$ by checking whether $t$ deprived of $\ell$ is an implicant of $T$ (which boils down to check whether $t$ intersects every clause of $\cnf(T)$ and
can be done in linear time). If so, remove $\ell$ from $t$ and proceed to the next literal.
Once all literals in $t_{\vec{x}}$ have been examined, the final term $t$ is by construction an implicant of $T$ such that
removing any literal from it would lead to a term that is not any longer an implicant of $T$. Thus, $t$
is a prime implicant of $T$ containing only literals from $\vec{x}$, alias a sufficient reason for $\vec x$ given $T$.
In the case of proto-sufficient reasons, the implicant test must be updated in such a way that $\ell$ is removed if and on if
$t$ deprived of $\ell$ is an implicant of a strict majority of trees in $F$. Of course, the greedy algorithm based on the updated 
implicant test runs in time polynomial in the size of the input. Note also that instead of starting it with $t = t_{\vec x}$, the greedy algorithm
can be run with $t = p_{\vec x}^F$ or, more generally, with any term $t$ such that $t \subseteq t_{\vec x}$ and 
$t$ an implicant of at least $\lfloor \frac{m}{2} \rfloor +1$ decision trees of $F$. Doing so, the correctness of the greedy algorithm
would not be questioned (and its efficiency could possibly be improved via less implicant tests).

Obviously enough, when $F$ consists of a single decision tree $T$, the proto-sufficient reasons for $\vec x$ given $F$ coincide with the 
sufficient reasons for $\vec x$ given $T$.

%\color{black}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Sufficient Reasons}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Another valuable notion of reason is the one of {\em sufficient reason}, defined for any Boolean classifier \cite{DarwicheHirth20}. Unlike direct reasons
and proto-sufficient reasons, sufficient reasons are ensured not to contain irrelevant characteristics, and as such, they can be considered as better explanations:

\begin{definition}[Sufficient Reason] 
    Let $f \in \mathcal F_n$ and $\vec x \in \{0,1\}^n$ such that $f(\vec x) = 1$.
       Then, a \emph{sufficient reason} for $\vec x$ given $f$ is a prime implicant $t$ of $f$ which covers $\vec x$.
\end{definition}

%\color{blue}

\begin{example} 
For our running example, $x_2 \wedge x_3 \wedge x_4$ and $x_1 \wedge x_4$ 
are the sufficient reasons for $\vec x$ given $F$.
%Based on our running example, $x_2 \wedge x_3 \wedge x_4$ 
%is a prime implicant of $F$ covering $\vec x$, and hence, a sufficient reason for $\vec x$ given $F$.
%It is better than $p_{\vec x}^F$ since it does not contain $x_1$ which is globally relevant but locally irrelevant ($F$ does not need
%this characteristics to classify $\vec x$ as it has been classified).
\end{example}

It is easy to show that the direct reason $p_{\vec x}^F$ for $\vec x$ given $F$ may contain arbitrarily many more features 
than a sufficient reason for $\vec x$ given $F$. Indeed, it has been shown recently that this is the case for decision trees \cite{DBLP:journals/corr/abs-2010-11034},
and the direct reason for an instance $\vec x$ given a random forest that contains a single tree $T$ coincides with the direct reason for $\vec x$ given $T$.
A similar result can be obtained for proto-sufficient reasons:

\begin{proposition} \label{prop:proto-sufficient}
Let $F = \{T_1, \ldots, T_m\}$ be a random forest of  $\rf_{n, m}$ and $\vec x \in \{0,1\}^n$ such that $F(\vec x) = 1$. Unless $m \geq 2$,
it can be the case that every proto-sufficient reason for $\vec x$ given $F$ contains arbitrarily many more features 
than any sufficient reason for $\vec x$ given $F$.
\end{proposition}

Actually, the notion of sufficient reason for $\vec x$ given a random forest appears as more tricky than the one for the case of decision trees. 
The greedy algorithm sketched above for computing sufficient reasons in the case of decision trees can still be used
for computing sufficient reasons given a random forest, but it must be based on an updated implicant test. Indeed, if 
$t$ an implicant of at least $\lfloor \frac{m}{2} \rfloor +1$ decision trees of $F$, then $t$ clearly is an implicant of $F$, but the
converse does not hold (otherwise, the notions of proto-sufficient reasons and of sufficient reasons would coincide, but this is
not the case as a by-product of Proposition \ref{prop:proto-sufficient}).
%
%Especially, though the implicant test for decision trees can be achieved efficiently, it is more complex in the case of random forests.
%
%Especially, in the case of a random 
%forest $F$, focusing on the sufficient reasons for $\vec x$ given the trees of $F$ is not enough to characterize  the sufficient 
%reasons for $\vec x$ given $F$. 
%More than that, focusing on the implicants $t$ of a majority of decision trees $T \in F$ such that $\vec x \models t$ holds 
%is not enough. As a matter of illustration, consider $F = \{T_1, T_2, 1\}$ where $T_1$ is a decision tree equivalent to $x_1 \wedge x_2$
%and $T_2$ is a decision tree equivalent to $x_1 \wedge \overline{x_2}$. $F$ is equivalent to $x_1$. The (unique) sufficient reason for 
%$\vec x = (1, 1)$ is $x_1$, but $x_1$ neither is an implicant of $t_1$ nor is an implicant of $T_2$.
%
%Nevertheless, two observations are worth being made: (1) the use of this greedy algorithm for generating sufficient reasons is not
%specific to decision trees, but it works for any Boolean classifier $f \in \mathcal F_n$ (possibly not in polynomial time,
%depending on the nature of $f$), and (2) the key test in this construction is the implicant one
%(testing whether a term is an implicant of $T$) that is iterated. This test is where the computational complexity of
%the greedy algorithm lies. For decision trees $T$, this test is quite simple and can be achieved in polynomial time (a consistent term $t$ is an implicant of 
%a decision tree $T$ when $t$ intersects every clause of $\cnf(T)$), and as a consequence, the greedy algorithm
%for deriving a sufficient reason for $\vec x$ given $T$ also runs in polynomial time. 
%
That mentioned, in the case of random forests, the implicant test can be achieved via a call
to a {\sc SAT} oracle:

\begin{proposition} \label{prop:implicanttestRF}
Let $F = \{T_1, \ldots, T_m\}$ be a random forest of  $\rf_{n, m}$. 
Let $t$ be a consistent term over $X_n$. Let $H$ be the \cnf\ formula 
$$\{(\overline y_i \vee c) : i \in [m], c \in \cnf(\neg T_i) \} \cup \cnf(\sum_{i = 1}^m y_i > \frac{m}{2})$$
where $\{y_1, \ldots, y_m\}$ are fresh variables and $\cnf(\sum_{i = 1}^m y_i > \frac{m}{2})$ is a \cnf\ encoding of the
cardinality contraint $\sum_{i = 1}^m y_i > \frac{m}{2}$. $t$ is an implicant of $F$ if and only if $t \wedge H$ is unsatisfiable.
\end{proposition}

Seemingly, one can hardly do better and design a polynomial-time algorithm for the implicant test, since this would imply that {\sf P = NP}: 

\begin{proposition} \label{prop:complexityimplicanttestRF}
    Let $F \in \rf_{n, m}$ and $\vec x \in \{0,1\}^n$ such that $F(\vec x) = 1$. 
    Let $t$ be a term over $X_n$ such that $t \subseteq t_{\vec x}$. Deciding whether $t$ is an implicant of $F$ is {\sf coNP}-complete.
\end{proposition}

%Interestingly, the {\sc SAT}-based implicant test for random forests given by Proposition \ref{prop:implicanttestRF} is only ``mildly hard''. 
Going one step further, the sufficient reasons for an instance $\vec x$ given a random forest $F$ can be characterized (and computed) in terms of
MUS (minimal unsatisfiable subsets). Given a set of clauses $S$ that is satisfiable and a set of clauses $H$ such that $S \cup H$ is unsatisfiable,
a MUS of $S$ given $H$ is a subset $I$ of clauses of $S$ such that $I \cup H$ is unsatisfiable, but for every clause $c \in I$, $(I \setminus \{c\}) \cup H$ 
is satisfiable. $H$ is a set of so-called hard clauses and $S$ (disjoint from $H$) contains the so-called soft clauses.  
A MUS is thus a subset $I$ of $S$ which is jointly unsatisfiable
with $H$ but becomes satisfiable with $H$ as soon as a single clause of $I$ is removed from $I$.
Note that one can assume without any loss of generality that 
$S = \{c_i : i \in \{1, \ldots, k\}\}$ is a set of literals (indeed, one can always replace $H$ by a \cnf\ formula $H' = H \cup \{\overline{y_i} \vee c_i : i \in \{1, \ldots, k\}\}$ 
and $S$ by $S' = \{y_1, \ldots, y_k\}$ in such a way that $I$ is a MUS of $S$ given $H$ if and only if 
$M' = \{y_i : c_i \in I\}$ is a MUS of $S'$ given $H'$).

\begin{proposition} \label{prop:sufficient reason-MUS-RF}
    Let $F \in \rf_{n, m}$ and $\vec x \in \{0,1\}^n$ such that $F(\vec x) = 1$. 
    Let $t$ be a term over $X_n$ such that $t \subseteq t_{\vec x}$. $t$ is a sufficient reason for $\vec x$ given $F$ if and only if
    $t$ is a MUS of $S= \{\ell : \ell \in t_{\vec x}\}$ given $H$, the \cnf\ formula given in Proposition \ref{prop:implicanttestRF}.
\end{proposition}

The characterization result given by Proposition \ref{prop:sufficient reason-MUS-RF} is valuable because many {\sc SAT}-based algorithms 
for computing a MUS (or even all MUSes) of a \cnf\ formula have been pointed out for the past decade \pierre{Ajouter des réfs ici.} One can take advantage of them for computing sufficient reasons (and this is what we did in our experiments). Note that when the objective is to compute a single sufficient reason for $\vec x$ given $F$ using
an algorithm for computing a MUS, we could consider $S = \{\ell : \ell \in p_{\vec x}^F\}$ 
or $S$ as the set of literals of any proto-sufficient reason for $\vec x$ given $F$ instead of considering $S = \{\ell : \ell \in t_{\vec x}\}$.

This time again, one can hardly expect to do much better and design a polynomial-time algorithm for computing a sufficient reason.
Indeed, as a consequence of Proposition \ref{prop:complexitysufficientreasonRF}, the tractability result about the generation of a sufficient reason 
for  $\vec x$ given a decision tree cannot be lifted to the more general case of a random forest, unless {\sf P = NP}.

\begin{proposition} \label{prop:complexitysufficientreasonRF}
    Let $F \in \rf_{n, m}$ and $\vec x \in \{0,1\}^n$ such that $F(\vec x) = 1$. 
    Deciding whether a term $t$ is a sufficient reason for  $\vec x$ given $F$ is {\sf DP}-complete.
    %in {\sf DP} and is both {\sf NP}-hard and {\sf coNP}-hard.
\end{proposition}

As a by-product of Proposition \ref{prop:complexitysufficientreasonRF}, using a MUS-based approach for computing 
a sufficient reason does not look as using a sledgehammer to crack a nut:
deciding whether $I$ is a MUS of $S$ given $H$ also is {\sf DP}-complete.
Furthermore, though the MUS-based algorithms to compute a sufficient reason do not run in polynomial time in the worst case, 
the tremendous progress in {\sc SAT} solving achieved for 
the past two decades, makes them quite practical in many cases  (see Section \ref{experiments}).

%\color{black}
%
%\newpage
%
%\fred{Preuves alternatives exploitant les resultats de Judy Goldsmith et ceux de Christopher Umans.}
%\pierre{Je mets en commentaires car cela a été ajouté plus loin via un \input}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Some Alternative Results}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%We first consider sufficient reasons for arbitrary propositional formulas.
%
%\begin{center}
%\fcolorbox{black}{white}
%{
%\begin{minipage}{0.98\textwidth}
%    \textsc{Is Prime Implicant (IPI)}
%    \begin{itemize}
%    \item \emph{Instance:} A Boolean formula $F$ and a monomial $t$.
%    \item \emph{Question:} Is $t$ a prime implicant of $F$?
%    \end{itemize}    
%\end{minipage}
%}
%\end{center}
%\vspace{0.5em}
%
%\begin{proposition}
%\textsc{Is Prime Implicant} is \textsf{DP}-complete.
%\end{proposition}
%\begin{proof}
%Directly follows from Theorem 5 in \cite{Goldsmith2008}.
%\end{proof}
%
%\begin{center}
%    \fcolorbox{black}{white}
%    {
%    \begin{minipage}{0.98\textwidth}
%        \textsc{Is Sufficient Reason (ISR)}
%        \begin{itemize}
%        \item \emph{Instance:} A Boolean formula $F$, an assignment $\vec x$, and a monomial $t$.
%        \item \emph{Question:} Is $t$ a sufficient reason of  $\vec x$ given $F$?
%        \end{itemize}    
%    \end{minipage}
%    }
%\end{center}
%\vspace{0.5em}
%    
%\begin{proposition}
%    \label{prop:ISR}
%\textsc{Is Sufficient Reason} is \textsf{DP}-complete.
%\end{proposition}
%\begin{proof}
%The membership part follows from the fact that ISR is a special case of IPI.
%For the hardness part, consider an instance $(F,t)$ of IPI, and let $(F,\vec x,t)$ be the corresponding 
%instance of ISR, where $\vec x$ is any assignment covered by $t$. Obvisouly, 
%$(F,\vec x,t)$ can be constructed in linear time. 
%Now, if $(F,t)$ is a solution of IPI, then $t$ is a prime implicant of $F$. This, 
%together with the fact that $t$ covers $\vec x$ implies that $(F,\vec x,t)$ is a solution of ISR.
%Conversely, if $(F,\vec x,t)$ is a solution of ISR, then $t$ is a a prime implicant of $F$, 
%which immediately implies that $(F,t)$ is a solution of IPI.  
%\end{proof}
%
%We now consider the subclass of DNF formulas.
%
%\begin{center}
%    \fcolorbox{black}{white}
%    {
%    \begin{minipage}{0.98\textwidth}
%        \textsc{Is DNF Prime Implicant (IPI[DNF])}
%        \begin{itemize}
%        \item \emph{Instance:} A DNF formula $F$ and a monomial $t$.
%        \item \emph{Question:} Is $t$ a prime implicant of $F$?
%        \end{itemize}    
%    \end{minipage}
%    }
%\end{center}
%\vspace{0.5em}
%
%\begin{proposition}
%    \textsc{Is DNF Prime Implicant} is \textsf{DP}-complete.
%\end{proposition}
%    \begin{proof}
%        Follows from Theorem 6.7 in \cite{Umans2006}.
%    \end{proof}
%    
%    \begin{center}
%        \fcolorbox{black}{white}
%        {
%        \begin{minipage}{0.98\textwidth}
%            \textsc{Is DNF Sufficient Reason (ISR[DNF])}
%            \begin{itemize}
%            \item \emph{Instance:} A DNF formula $F$, an assignment $\vec x$, and a monomial $t$.
%            \item \emph{Question:} Is $t$ a sufficient reason of  $\vec x$ given $F$?
%            \end{itemize}    
%        \end{minipage}
%        }
%    \end{center}
%    \vspace{0.5em}
%
%\begin{proposition}
%        \textsc{Is DNF Sufficient Reason} is \textsf{DP}-complete.
%        \end{proposition}
%        \begin{proof}
%          Straightforward, using a strategy similar to the proof of Proposition \ref{prop:ISR}.  
%        \end{proof}
%
%With these results in hand, let us turn to our problem.
%
%\begin{center}
%    \fcolorbox{black}{white}
%    {
%    \begin{minipage}{0.98\textwidth}
%        \textsc{Is Sufficient Reason for Random Forests (ISR[RF])}
%        \begin{itemize}
%        \item \emph{Instance:} A random forest $F$, an assignment $\vec x$, and a monomial $t$.
%        \item \emph{Question:} Is $t$ a sufficient reason of  $\vec x$ given $F$?
%        \end{itemize}    
%    \end{minipage}
%    }
%\end{center}
%\vspace{0.5em}
%
%\begin{proposition}
%\textsc{Is Sufficient Reason} is \textsf{DP}-complete.
%\end{proposition}
%\begin{proof}
%    The membership part follows from the fact that ISR[RF] is a special case of ISR, and the hardness 
%    part follows from the fact that ISR[DNF] is a special case of ISR[RF].
%\end{proof}
%    

%For illustration, the following toy example will be used throughout the paper as a running example:


% Deciding whether any term $t$ included in $\vec x$ is an implicant of $T$ is equivalent to checking whether 
% $t$ entails $\cnf(T)$, which can be done in $O(\size{T})$ time. 
% Thus, by performing this implicant test $n$ times, the runtime of the greedy algorithm is in $\mathcal O(\size{T}n)$.

% The key task of the greedy algorithm is to decide whether any term $t$ included in $\vec x$  is an 
% implicant of $T$, which is equivalent to check whether $T \mid t$ (the conditioning of $T$ by $t$) 
% is a decision tree with no leaves labeled by $0$. To this point, $T \mid t$ can be constructed in $O(\size{T})$
% time using the following procedure: sort all internal vertices of $T$ in reverse topological order and, 
% for each vertex $v_i$ in that order, check whether the corresponding variable $x_i$ 
% occurs as a literal $l_i$ of $t$\footnote{This can be done in $\mathcal O(1)$ time using a vector encoding of $t$.}. 
% If so, replace the node $v_i$ by its right child if $l_i = x_i$, and its left child if $l_i = \overline x_i$.
% By performing this implicant test $n$ times, the runtime of the greedy algorithm is in $\mathcal O(\size{T}n)$.

% which returns as output a sufficient reason $t$ for $\vec x$ given $T$ in $\mathcal O(n \size{T})$ time.
% \footnote{Note that this algorithm can be extended easily to the case of random forests without questioning its tractability.}
% The tractability of finding sufficient reasons in decision trees lies in the fact that deciding whether a consistent term $t$ is an implicant 
% of a decision tree $T$ can be obtained by checking whether $T \mid t$ (the conditioning of $T$ by $t$) 
% is a decision tree with no leaves labeled by $0$. Notably, $T \mid t$ can be computed in $\mathcal O(\size{T} \size{t})$ 
% time by iteratively conditioning $T$ by each literal occurring in $t$. For any such literal $l_i$ with variable $x_i$,
% $T \mid l_i$ is obtained by simply replacing each internal node $x_i$ in $T$ with its right child if $l_i = x_i$, 
% and its left child if $l_i = \overline x_i$.
    % With this implicant test in hand, the generation of a sufficient reason for $\vec x$ given $T$ 
% can be found using the following greedy algorithm: start with $t = \vec x$, and iterate over the literals $l_i$ of 
% $t$ by checking whether $t$ deprived of $l_i$ is still an implicant of $T$. 
% If so, remove $l_i$ from $t$ and proceed to the next literal.
% Once all the variables $\vec{x}$ have been examined, the term $t$ is by construction an implicant of $T$ such that
% removing any literal from $t$ would lead to a term that is not any longer an implicant of $T$. Thus, $t$
% is a prime implicant of $T$ and it contains only literals from $\vec{x}$.


% Deciding whether any term $t$ included in $\vec x$ is an implicant of $T$ is equivalent to checking whether 
% $t$ entails $\cnf(T)$, which can be done in $O(\size{T})$ time. 
% Thus, by performing this implicant test $n$ times, the runtime of the greedy algorithm is in $\mathcal O(\size{T}n)$.

% The key task of the greedy algorithm is to decide whether any term $t$ included in $\vec x$  is an 
% implicant of $T$, which is equivalent to check whether $T \mid t$ (the conditioning of $T$ by $t$) 
% is a decision tree with no leaves labeled by $0$. To this point, $T \mid t$ can be constructed in $O(\size{T})$
% time using the following procedure: sort all internal vertices of $T$ in reverse topological order and, 
% for each vertex $v_i$ in that order, check whether the corresponding variable $x_i$ 
% occurs as a literal $l_i$ of $t$\footnote{This can be done in $\mathcal O(1)$ time using a vector encoding of $t$.}. 
% If so, replace the node $v_i$ by its right child if $l_i = x_i$, and its left child if $l_i = \overline x_i$.
% By performing this implicant test $n$ times, the runtime of the greedy algorithm is in $\mathcal O(\size{T}n)$.

% which returns as output a sufficient reason $t$ for $\vec x$ given $T$ in $\mathcal O(n \size{T})$ time.
% \footnote{Note that this algorithm can be extended easily to the case of random forests without questioning its tractability.}
% The tractability of finding sufficient reasons in decision trees lies in the fact that deciding whether a consistent term $t$ is an implicant 
% of a decision tree $T$ can be obtained by checking whether $T \mid t$ (the conditioning of $T$ by $t$) 
% is a decision tree with no leaves labeled by $0$. Notably, $T \mid t$ can be computed in $\mathcal O(\size{T} \size{t})$ 
% time by iteratively conditioning $T$ by each literal occurring in $t$. For any such literal $l_i$ with variable $x_i$,
% $T \mid l_i$ is obtained by simply replacing each internal node $x_i$ in $T$ with its right child if $l_i = x_i$, 
% and its left child if $l_i = \overline x_i$.
    % With this implicant test in hand, the generation of a sufficient reason for $\vec x$ given $T$ 
% can be found using the following greedy algorithm: start with $t = \vec x$, and iterate over the literals $l_i$ of 
% $t$ by checking whether $t$ deprived of $l_i$ is still an implicant of $T$. 
% If so, remove $l_i$ from $t$ and proceed to the next literal.
% Once all the variables $\vec{x}$ have been examined, the term $t$ is by construction an implicant of $T$ such that
% removing any literal from $t$ would lead to a term that is not any longer an implicant of $T$. Thus, $t$
% is a prime implicant of $T$ and it contains only literals from $\vec{x}$.
%
%Finally, it is worth noting that the problem of deriving \emph{all} sufficient reasons for
%a given instance is much more demanding in general. Indeed, even for the restricted class of decision trees with
%logarithmic depth, an input instance can have exponentially many sufficient reasons:
%
%\begin{proposition}\label{prop:nbDT}
%%    Let $\dt^k_{n}$ be the class of decision trees of depth $k \geq 1$ over $n = 2^k - 1$ variables. Then, t
%There is a decision tree $T$ of depth $k \geq 1$ over $n = 2^k - 1$ variables
% such that for any $\vec x \in \{0,1\}^n$, the number of sufficient reasons for $\vec x$ given $T$ is at least 
% $\lfloor \frac{3}{2}^{\frac{n + 1}{2}} \rfloor$. 
%\end{proposition}

